Non-Convex Optimizations for Machine Learning with Theoretical Guarantee: Robust Matrix Completion and Neural Network Learning

Despite the recent development in machine learning, most learning systems are still under the concept of "black box", where the performance cannot be understood and derived. With the rise of safety and privacy concerns in public, designing an explainable learning system has become a new trend in machine learning. In general, many machine learning problems are formulated as minimizing (or maximizing) some loss function. Since real data are most likely generated from non-linear models, the loss function is non-convex in general. Unlike the convex optimization problem, gradient descent algorithms will be trapped in spurious local minima in solving non-convex optimization. Therefore, it is challenging to provide explainable algorithms when studying non-convex optimization problems. In this thesis, two popular non-convex problems are studied: (1) low-rank matrix completion and (2) neural network learning.

==> chapter_1/analysis_publication_ready.tex <==
\section*{Appendix }
\subsection{Notations and assumptions}

We first introduce notations used in the proof. 
For matrix $\bfZ_1\in\mathbb{C}^{n_c\times n}$, we define the \textbf{Block Hankel Operator} $\widetilde{\mathcal{H}}$ as
\vspace{-1mm}
$$\widetilde{\mathcal{H}}\bfZ_1
\vspace{-1mm}
=\begin{bmatrix}
\mathcal{H}\bfZ_1&\mathcal{H}\bfZ_1&\cdots&\mathcal{H}\bfZ_1
\end{bmatrix}
\in\mathbb{C}^{n_cn_1\times n_cn_2}.$$
$\widetilde{\mathcal{H}}\bfZ_1$ is an $n_c$-block Hankel matrix.
 $\widetilde{\mathcal{H}}^*$ is the adjoint operator of $\widetilde{\mathcal{H}}$. For any matrix $\bfZ_2\in \mathbb{C}^{n_cn_1\times n_cn_2}$, $(\widetilde{\mathcal{H}}^*\bfZ_2)\in\mathbb{C}^{n_c\times n}$ satisfies
\vspace{-3mm}
\begin{equation*}
\langle\widetilde{\mathcal{H}}^*\bfZ_2,\bfe_k \bfe_t^*\rangle=\sum_{l=0}^{n_c-1}\sum_{k_1+k_2=t+1}\langle\bfZ, \bfe_{(k_1-1)n_c+k}\bfe_{k_2+ln_2}^*\rangle.
\end{equation*}
Define  $\mathcal{\widetilde{D}}^2:=\widetilde{\mathcal{H}}^*\mathcal{\widetilde{H}}$, an operator from an $n_c\times n$ matrix $\bfZ$ to an $n_c \times n$ matrix with $$\widetilde{\mathcal{D}}^2\bfZ=\sum_{t=1}^{n}\sum_{k=1}^{n_c}n_cw_t\langle{\bfZ},\bfe_{k}\bfe_{t}^*\rangle\bfe_{k}\bfe_{t}^*,$$ 
where $w_t$ is defined in \eqref{w}. Then the Moore-Penrose pseudoinverse of $\widetilde{\mathcal{H}}$, denoted as $\widetilde{\mathcal{H}}^{\dagger}$, equals to $\widetilde{\mathcal{D}}^{-2}\widetilde{\mathcal{H}}^*$.  Further, we define $\mathcal{\widetilde{G}}=\mathcal{\widetilde{H}}\mathcal{\widetilde{D}}^{-1},$ then the adjoint operator of $\mathcal{\widetilde{G}}$ is defined as $\mathcal{\widetilde{G}}^*=\mathcal{\widetilde{D}}^{-1}\mathcal{\widetilde{H}}^*$. 
Additionally,
%\vspace{-1mm}
\begin{equation}\label{y_l}
\vspace{-1mm}
\bfY :=\widetilde{\mathcal{D}}{\bfX} \quad \text{and} \quad {\bfY}_l:=\widetilde{\mathcal{D}}{\bfX}_l.
\end{equation}
 
For any matrix $\bfZ\in\mathbb{C}^{n_c\times n}$, one can check that $ \| \widetilde{\mathcal{H}}{\bfX}\|=\sqrt{n_c}\left\| {\mathcal{H}}{\bfX}\right\|$ and $\| \widetilde{\mathcal{H}}{\bfX}\|_F=\sqrt{n_c}\left\| {\mathcal{H}}{\bfX}\right\|_F $. Immediately, 
$\widetilde{\mathcal{H}}\bfX$ and ${\mathcal{H}}\bfX$ share the same conditional number $\kappa$. Moreover, it is clear that $\widetilde{\mathcal{G}}$ is a unit operator as $\mathcal{\widetilde{G}}^*\mathcal{\widetilde{G}}=\mathcal{{I}}$, and $\mathcal{\widetilde{H}}{\bfX}=\mathcal{\widetilde{G}}{\bfY}$.


%\begin{itemize}
%	\item $\mathcal{\widetilde{G}}^*\mathcal{\widetilde{G}}=\mathcal{{I}}, \left\|\mathcal{\widetilde{G}}\right\|= 1 $ and $\left\|\mathcal{\widetilde{G}}^*\right\|= 1$;
%	\item $\mathcal{\widetilde{G}}{\bfZ}=\displaystyle\sum_{t=1}^{n}\sum_{k=1}^{n_c}\langle{\bfZ},\bfe_{k}\bfe_{t}^*\rangle\widetilde{{\bfH}}_{k,t}, \forall {\bfZ}\in \mathbb{C}^{n \times n_c};$
%	\item $\mathcal{\widetilde{G}}^*{\bfZ}=\displaystyle\sum_{t=1}^{n}\sum_{k=1}^{n_c}\langle{\bfZ},\widetilde{{\bfH}}_{k,t}\rangle\bfe_{k}\bfe_{t}^*$, $\forall {\bfZ}\in \mathbb{C}^{n_cn_1\times n_cn_2}.$
%\end{itemize}
The following proofs will be established on Block Hankel Operator $\widetilde{\mathcal{H}}$. Consider AM-FIHT in terms of $\widetilde{\mathcal{H}}$,
the initialization can be written as  $\widetilde{{\bfL}}_0=p^{-1}\mathcal{Q}_r(\widetilde{{\mathcal{H}}}\mathcal{P}_{\Omega}({\bfX}))$. Further, the major steps can be represented as
\vspace{-1mm}
\begin{equation*}
\vspace{-2mm}
\widetilde{{\bfW}}_l=\mathcal{P}_{\widetilde{{\bf\mathcal{S}}}_l}\widetilde{\mathcal{H}}({\bfX}_l+p^{-1}{\bfG}_l+\beta\Delta\widetilde{\bfW}),\quad \widetilde{{\bfL}}_{l+1}=\mathcal{Q}_r(\widetilde{{\bfW}}_l),
\end{equation*}
where $\widetilde{\mathcal{{\bfS}}}_l$ is the tangent subspace at $\widetilde{{\bfL}}_l$. The resulting $\widetilde{\bfX}_l$ returned by AM-FIHT in terms of $\widetilde{\mathcal{H}}$ is given as $\widetilde{\mathcal{H}}^{\dagger}\widetilde{\bfL}_{l}$. 

Moreover, by replacing $\mathcal{H}$ with $\widetilde{\mathcal{H}}$,  AM-FIHT returns the same result as $\widetilde{\bfX}_l=\bfX_l$. In other words, 
we can show  that 
\begin{equation}\label{bar}
\widetilde{{\bfL}}_l=\begin{bmatrix}
{\bfL}_l &{\bfL}_l &\cdots &{\bfL}_l
\end{bmatrix}, \forall l\ge0.
\end{equation}
%A brief proof is followed. 
%\begin{proof}
To see this, it is clear that (\ref{bar}) holds for $l=0$ from the definition of $\widetilde{\bfL}_0$.	Then suppose (\ref{bar}) holds when $l=k$. Immediately, we have $\widetilde{{\bfW}}_{k}=\begin{bmatrix}
	{\bfW}_{k} &{\bfW}_{k} &\cdots &{\bfW}_{k}
	\end{bmatrix}$. Let  ${\bfW}_{k}=\sum_{i=1}^{\min(n_cn_1, n_2)}\sigma_i {\bfu}_i{\bfv}_i^*$ be the SVD with $\sigma_1\ge\sigma_2\ge\cdots\ge\sigma_{\min(n_cn_1, n_2)}$.  Then for $l=k+1$, 
	\small
	\vspace{-2mm}
	\begin{equation*}
	\vspace{-2mm}
	\begin{split}
	\widetilde{{\bfL}}_{k+1}=\mathcal{Q}_r(\widetilde{{\bfW}}_{k})
	&=\sum_{i=1}^{r}\sqrt{n_c}\sigma_i {\bfu}_i \frac{1}{\sqrt{n_c}}
	\begin{bmatrix}
	{\bfv}_i^*& \cdots& {\bfv}_i^*
	\end{bmatrix}\\
	&=\sum_{i=1}^{r}\begin{bmatrix}
	\sigma_i {\bfu}_i{\bfv}_i^*& \cdots& \sigma_i {\bfu}_i{\bfv}_i^*
	\end{bmatrix}.\\
	&=\begin{bmatrix}
	{\bfL}_{k+1} &{\bfL}_{k+1} &\cdots &{\bfL}_{k+1}
	\end{bmatrix}.
	\end{split}
	\end{equation*}
	\normalsize
Hence, the connection between $\bfX_l$ and $\widetilde{\bfL}_l$ can be given as 
\begin{equation}
\begin{split}
&\|\bfX_l-\bfX\|_F
=\|\widetilde{\mathcal{D}}^{-1}({\bfY}_l-{\bfY})\|_F\le \frac{1}{\sqrt{n_c}}\|{\bfY}_l-{\bfY}\|_F\\
&~~~=\frac{1}{\sqrt{n_c}}\|\widetilde{\mathcal{G}}^{*}(\widetilde{\bfL}_l-\widetilde{\mathcal{G}}{\bfY})\|_F\le \frac{1}{\sqrt{n_c}}\|\widetilde{\bfL}_l-\widetilde{\mathcal{G}}{\bfY}\|_F.
\end{split}
\end{equation}


For RAM-FIHT, 
similarly define an $n_c$-block matrix 
 $\widetilde{\bfL}^{\prime}_l=\begin{bmatrix}
\bfL^{\prime}_l&\bfL^{\prime}_l&\cdots&\bfL^{\prime}_l
\end{bmatrix}$. From the discussion above, one can verify that (\ref{bar}) also holds in RAM-FIHT. Then 
the SVD of $\widetilde{\bfL}_l$ in \eqref{bar} is $\widetilde{\bfL}_l=\widetilde{\bfU}_l\widetilde{\bf\Sigma}_l\widetilde{\bfV}_l^*
=
\bfU_l \big(\sqrt{n_c}{\bf\Sigma}_l\big)
\big(\frac{1}{\sqrt{n_c}}[\bfV_l^* \cdots \bfV_l^*]
\big)$. Then $\widetilde{\bfA}_l$ and $\widetilde{\bfB}_l$ are defined as 
\small
\begin{equation}\label{trimming1}
(\widetilde{\bfA}_{l})_{i*}=\displaystyle\frac{(\widetilde{\bfU}_{l})_{i*}}{\left\| (\widetilde{\bfU}_{l})_{i*}\right\|}\min\bigg\{\left\|(\widetilde{\bfU}_{l})_{i*} \right\|, \sqrt{\frac{\mu r}{n_cn_1}} \bigg\},
\end{equation}
\begin{equation}\label{trimming2}
(\widetilde{\bfB}_{l})_{i*}=\displaystyle\frac{(\widetilde{\bfV}_{l})_{i*}}{\left\| (\widetilde{\bfV}_{l})_{i*}\right\|}\min\bigg\{\left\|(\widetilde{\bfV}_{l})_{i*} \right\|, \sqrt{\frac{\mu r}{n_cn_2}} \bigg\}.
\end{equation}
\normalsize

{\bf Sampling model with replacement}. As shown in  \cite{R11}, %it adopted the sampling model with replacement, which leaded to a simpler analysis because of the independence of entries.
due to the duplications,  %As the duplicate entries in sampling model with replacement,
 the number of observed entries in a sampling model with replacement is less than or equal to that in a sampling model without replacement. %Hence, to achieve the same probability of successful recovery, the size of $\Omega$ under sampling model without replacement should be less than the one under sampling model with replacement. Therefore, 
 Thus, it is sufficient to study the sampling model with replacement. %$\Omega$ is based on the sampling model with replacement. 
 To distinguish $\widehat{\Omega}$ in \eqref{m2}, which represents the sampling set without replacement, let $\Omega$ be $m$ unions of indices sampled uniformly from set $\{1,2,\cdots,n_c\}\times\{1,2,\cdots,n\}$ with replacement, and
 \vspace{-2mm}
 \begin{equation}\label{sampling with replacement}
 \vspace{-2mm}
 \mathcal{P}_{\Omega}(\bfZ_1)=\sum_{a=1}^{m}\langle\bfZ_1, \bfe_{k_a}\bfe_{t_a}^*\rangle\bfe_{k_a}\bfe_{t_a}^*,
 \end{equation}
%  since $\Omega$ may have repetitive elements. In this case, $\mathcal{P}_{\Omega}$ is no longer a projection since $\mathcal{P}_{\Omega}\mathcal{P}_{\Omega}\ne\mathcal{P}_{\Omega}$.
 for any $\bfZ_1\in\mathbb{C}^{n_c\times n}$. By changing the sampling model, several critical lemmas can be derived from Bernstein Inequality.
\begin{lemma}[\cite{T12}, Theorem 1.6]\label{prob}
	Consider a finite sequence $\{{\bfZ}_k\}$ of independent, random matrices with dimensions $d_1\times d_2$. Assume that such random matrix satisfies
	\vspace{-2mm}
	\begin{equation*}
	\vspace{-2mm}
	\mathbb{E}({\bfZ_k})=0\quad and \quad \left\|{\bfZ_k}\right\|\le R \quad almost ~ surely.	
	\end{equation*}
	Define
	\vspace{-2mm}
	\begin{equation*}
	\vspace{-2mm}
	\sigma^2:=\max\Big\{\Big\|\sum_{k}\mathbb{E}({\bfZ}_k{\bfZ}_k^*)\Big\|,\Big\|\displaystyle\sum_{k}\mathbb{E}({\bfZ}_k^*{\bfZ}_k)\Big\|\Big\}.
	\end{equation*}
	Then for all $t\ge0$,
	\begin{equation*}
	\mathbb{P}\Bigg\{ \left\|\displaystyle\sum_{k}{\bfZ}_k\right\|\ge t \Bigg\}\le(d_1+d_2)\exp\Big(\frac{-t^2/2}{\sigma^2+Rt/3}\Big).
	\end{equation*}
\end{lemma}
Suppose that $t\le \sigma^2/R$, then the right hand side can be released as $(d_1+d_2)\exp(-\frac{3}{8}t^2/\sigma^2)$. Such kind of manipulation will be adopted in several proofs.

Note that the set of matrices $$\big\{\widetilde{{\bfH}}_{k.t}|\widetilde{{\bfH}}_{k,t}=\frac{1}{\sqrt{n_cw_t}}\widetilde{\mathcal{H}}({\bfe}_k{\bfe}_t^*),1\le k \le n_c, 1\le t \le n\big\}$$ forms an orthonormal basis of the $n_c$-block Hankel matrix, where
$\widetilde{\mathcal{H}}\bfX=\sum_{k=1}^{n_c}\sum_{t=1}^{n}\langle\widetilde{{\bfH}}_{k,t}, \widetilde{\mathcal{H}}\bfX\rangle\widetilde{{\bfH}}_{k,t}$. Then, for all $(k_a,t_a)\in\Omega$, $\mathcal{P}_{\Omega}$ is also used as the operator
 \begin{equation*}
 \mathcal{P}_{\Omega}({\bfZ}_2)=\sum_{a=1}^{m}\langle{\bfZ}_2,\widetilde{{\bfH}}_{k_a,t_a}\rangle\widetilde{{\bfH}}_{k_a,t_a},
 \end{equation*}
 for any ${\bfZ}_2\in\mathbb{C}^{n_cn_1 \times n_cn_2}$. In spite of abuse of notation, the meaning of $\mathcal{P}_{\Omega}$ is clear from context. By such definition,  $\mathcal{P}_{\Omega}(\widetilde{\mathcal{H}}{\bfZ}_1)=\widetilde{\mathcal{H}}\mathcal{P}_{\Omega}({\bfZ}_1)$ for any ${\bfZ}_1\in\mathbb{C}^{n \times n_c}$. Additionally,
$\widetilde{{\bfH}}_{k,t}$ only has $n_c{w}_t$ nonzero entries of magnitude $1/\sqrt{n_c{w}_t}$, so $\|\widetilde{{\bfH}}_{k,t} \|_F =1$. The following lemma can be established directly from the definition of incoherence.
\begin{lemma}\label{def}
	Let $\mathcal{\widetilde{H}}{\bfX}={\widetilde{\bfU}\widetilde{\bf\Sigma} \widetilde{\bfV}^*}$ be the SVD of $\widetilde{\mathcal{H}}\bfX$. Assume $\mathcal{\widetilde{H}}{\bfX}$ is $\mu$-incoherent. Then\\
	\begin{equation}\label{co_1}
	\left\|{\bfe}_{k_1}^*\widetilde{{\bfU}}\right\|^2\le\frac{\mu c_sr}{n_cn} \quad, \quad \left\| {\bfe}_{k_2}^*\widetilde{{\bfV}}\right\|^2\le\frac{\mu c_sr}{n_cn},
	\end{equation}
	\begin{equation}\label{co_2}
	\left\|\mathcal{P}_{\widetilde{{\bfU}}}(\widetilde{{\bfH}}_{k,t})\right\|_F^2\le \displaystyle\frac{\mu c_sr}{n_cn} \quad ,\quad   \left\|\mathcal{P}_{\widetilde{{\bfV}}}(\widetilde{{\bfH}}_{k,t})\right\|_F^2\le \displaystyle\frac{\mu c_sr}{n_cn}.
	\end{equation}
	where ${\bfe}_{k_1},{\bfe}_{k_2}$ are the coordinate unit vectors.
\end{lemma}

%The proof of $(\ref{co_1})$ is trivial. To obtain $(\ref{co_2})$, we use $$\|\mathcal{P}_{\widetilde{{\bfU}}}(\widetilde{{\bfH}}_{k,t})\|_F^2=\langle\widetilde{{\bfU}}\widetilde{{\bfU}}^*, \widetilde{{\bfH}}_{k,t}\widetilde{{\bfH}}_{k,t}^*\rangle\le \| \widetilde{{\bfU}}\widetilde{{\bfU}}^*\| _{\infty}\|\widetilde{{\bfH}}_{k,t} \|_F^2.$$ 


==> chapter_1/proof_coherent_publication_ready.tex <==
\vspace{-5mm}
\subsection{Proof of Theorem \ref{coherent}}
We first introduce some useful lemmas. % to complete the proof of Theorem \ref{coherent}.
\begin{lemma}[\cite{HJ85}, Corollary 7.7.4(a)]\label{matrix}
	If ${\bfA},{\bfB}\in\mathbb{C}^{n}$ are positive-definite, then ${\bfA}\succeq{\bfB}$ if and only if ${\bfB}^{-1}\succeq{\bfA}^{-1}$
\end{lemma}
\begin{lemma}[\cite{MK04}, Theorem 7]\label{msp}
	Let $\lambda_1\ge\cdots\ge\lambda_n$ be eigenvalues of ${\bfA}$, denoted by $\lambda_i({\bfA})=\lambda_i$. 
	Let ${\bfA}$ and ${\bfB}$ be Hermitian positive semi-definite $n \times n$ matrices. If
	$1\le k \le i\le n$ and $1\le l \le n-i+1 $, then 
	\vspace{-1mm}
	\begin{equation*}
	\vspace{-1mm}
	\lambda_{i+l-1}({\bfA})\lambda_{n-l+1}({\bfB})\le \lambda_i({\bfA\bfB})\le \lambda_{i-k+1}({\bfA})\lambda_{k}({\bfB}).
	\end{equation*}
	In particular,
%	\vspace{-1mm}
%	\begin{equation*}
%	\vspace{-1mm}
%	\lambda_{i}({\bfA})\lambda_{n}({\bfB})\le \lambda_i({\bfA\bfB})\le \lambda_{i}({\bfA})\lambda_{1}({\bfB}).
%	\end{equation*}
%	and further
	\vspace{-1mm}
	\begin{equation*}
	\vspace{-1mm}
	\lambda_n({\bfA})\lambda_n({\bfB})\le\lambda_n({\bfA\bfB}), \quad
	\lambda_1({\bfA\bfB})\le\lambda_1({\bfA})\lambda_1({\bfB}).
	\end{equation*}
\end{lemma}

\begin{proof}[Proof of Theorem \ref{coherent}]
	 Consider $n_c=1$, the definition of $\mathcal{H}$ can be extended to a row vector, which corresponds with one channel data. Let $\mathcal{H}\bfX_{k*}=\bfU_k{\bf\Sigma}_k{\bfV}_k$ and $\mathcal{H}\bfX=\bfU{\bf\Sigma}{\bfV}$ be the SVD of $\mathcal{H}\bfX_{k*}$ and $\mathcal{H}\bfX$. Then, $\mu_0$ is defined as
	 \vspace{-1mm}
	\begin{equation*}
	\vspace{-1mm}
	\max_{k_1}\left\|{\bfe}_{k_1}^*{\bfU}_k\right\|^2\le\frac{\mu_0 r}{n_1}, \quad 
	\max_{k_2}\left\|{\bfe}_{k_2}^*{\bfV}_k\right\|^2\le\frac{\mu_0 r}{n_2}.
	\end{equation*}
	Notice that all $\mathcal{H}\bfX_{k*}$ share the same column space and row space, they have the same incoherence $\mu_0$. 
	It is trivial $\mu=\mu_0$ if we consider the incoherence of row spaces. Hence, we only focus on the incoherence of column space.
	
	By (\ref{Hankel X}), $\mathcal{H}\bfX=\bfP_L{\bf\Gamma}\bfP_R^T$. 
%	Let $\bfC=[\bfc_1,\cdots,\bfc_{n_c}]^*$.
	Define a series of diagonal matrices ${\bfD}_k$ as ${\bfD}_k=\text{diag}({\bfd}_{k})$ with $1\le k\le n_c$, and ${\bfd}_k=[d_{k,1},\cdots,  d_{k,r}]$, where $d_{k,i}=\bfr_i^*\bfs_1\bfC_{k*}\bfl_i$. We need one mild assumption that $d_{k,i}\ne0$. It guarantees that each ${\bfD}_k$ is full rank. Thus, $\mathcal{H}\bfX_{k*}=\bfE_L\bfD_k\bfP_R$, where $\bfE_L=\bfP_L$ with $n_c=1$. There exists a row-switching matrix $\bfQ_1$ satisfying
	\small
	\begin{equation*}
	\bfQ_1(\mathcal{H}\bfX)=\begin{bmatrix}
	\mathcal{H}\bfX_{1*}\\
	\mathcal{H}\bfX_{2*}\\
	\vdots\\
	\mathcal{H}\bfX_{n_c*}
	\end{bmatrix}=\begin{bmatrix}
	\bfE_L\bfD_1\\
	\bfE_L\bfD_2\\
	\vdots\\
	\bfE_L\bfD_{n_c}
	\end{bmatrix}\bfP_R:=\widetilde{\bfE}_L\bfP_R.
	\end{equation*}
	\normalsize
	Define a mapping $f:\{1,2,\cdots,n_cn_1\}\mapsto\{1,2,\cdots,n_cn_1\}$, $f(z)=w$ with $\bfe_z=\bfQ_1\bfe_w$, then $f$ is a bijective mapping.
%	${{\bfU}}$ can be written as ${{\bfU}}=\widetilde{{\bfE}}_L(\widetilde{{\bfE}}_L^*\widetilde{{\bfE}}_L)^{-1/2}{\bfQ_2}$ with orthogonal columns, where ${\bfQ_2}\in\mathbb{C}^{r\times r} $ is an orthonormal matrix. 
	Hence, we have
	\small
	\begin{equation}\label{pom}
	\vspace{-2mm}
	\begin{split}
	&\max_{l_1}\left\|{\bfe}_{l_1}^*{{\bfU}}\right\|^2
%	&=\left\|{\bfe}_{k_1}^*\widetilde{{\bfE}}_L(\widetilde{{\bfE}}_L^*\widetilde{{\bfE}}_L)^{-1/2}{\bfQ_2}\right\|^2\\
	=\max_{ k_1}(\bfQ_1{\bfe}_{k_1})^*\widetilde{{\bfE}}_L(\widetilde{{\bfE}}_L^*\widetilde{{\bfE}}_L)^{-1}\widetilde{{\bfE}}_L^*(\bfQ_1{\bfe}_{k_1})\\
	&=\max_{k_1}{\bfe}_{k_1}^*\widetilde{{\bfE}}_L\left(\sum_{k=1}^{n_c}{\bfD}_k^*{\bfE}_L^*{\bfE}_L{\bfD}_k\right)^{-1}\widetilde{{\bfE}}_L^*{\bfe}_{k_1}.	
	\end{split}
	\end{equation}
	\normalsize
	Consider $1\le k_1\le n_1$,  we know that ${\bfe}_{k_1}^*\widetilde{{\bfE}}_L=\widehat{{\bfe}}_{k_1}^*{\bfE}_L{\bfD}_1$, where ${\bfe}_{k_1} \in \mathbb{C}^{n_cn_1}$ and $\widehat{{\bfe}}_{k_1} \in \mathbb{C}^{n_1}$ are both coordinate vectors. Additionally, it is easy to show that symmetric matrices $\{{\bfD}_k^*{\bfE}_L^*{\bfE}_L{\bfD}_k\}_{k=1}^{n_c}$ are positive definite since $\{{\bfE}_L{\bfD}_k\}_{k=1}^{n_c}$ are full rank. Also, following Lemma \ref{matrix}, we have 
	\small
	\begin{equation}\label{S_ps}
	\begin{split}
	\sum_{k=1}^{n_c}{\bfD}_k^*{\bfE}_L^*{\bfE}_L{\bfD}_k& \succ{\bfD}_1^*{\bfE}_L^*{\bfE}_L{\bfD}_1\succ 0,\\
	\Big(\sum_{k=1}^{n_c}{\bfD}_k^*{\bfE}_L^*{\bfE}_L{\bfD}_k\Big)^{-1}&\prec({\bfD}_1^*{\bfE}_L^*{\bfE}_L{\bfD}_1)^{-1}.
	\end{split}	
	\end{equation}
%	where $\bfA\succ\bfB$ means $\bfA-\bfB$ is positive definite. 
%Following Lemma \ref{matrix}, we have
%	Due to Lemma \ref{matrix} and the fact that the inverse of any nonsingular matrix is unique, we have % We can extend it to strict case as
%	\begin{equation}\label{S_ps}
%	\Big(\sum_{k=1}^{n_c}{\bfD}_k^*{\bfE}_L^*{\bfE}_L{\bfD}_k\Big)^{-1}\prec({\bfD}_1^*{\bfE}_L^*{\bfE}_L{\bfD}_1)^{-1}.
%	\end{equation}
%	\normalsize
%	Thus, 
	\small
	\vspace{-3mm}
	Then,
	\begin{equation*}
	\begin{split}
	\left\|{\bfe}_{k_1}^*{{\bfU}}\right\|^2
	&=\widehat{{\bfe}}_{k_1}^*{\bfE}_L{\bfD}_1\Big(\sum_{k=1}^{n_c}{\bfD}_k^*{\bfE}_L^*{\bfE}_L{\bfD}_k\Big)^{-1}{\bfD}_1^*{\bfE}_L^*\widehat{{\bfe}}_{k_1}\\
	&<\widehat{{\bfe}}_{k_1}^*{\bfE}_L{\bfD}_1({\bfD}_1^*{\bfE}_L^*{\bfE}_L{\bfD}_1)^{-1}{\bfD}_1^*{\bfE}_L^*\widehat{{\bfe}}_{k_1}\\
%	&=\widehat{{\bfe}}_{k_1}^*{\bfE}_L{\bfD}_1{\bfD}_1^{-1}({\bfE}_L^*{\bfE}_L)^{-1}{\bfD}_1^{-*}{\bfD}_1^*{\bfE}_L^*\widehat{{\bfe}}_{k_1}\\
	&=\widehat{{\bfe}}_{k_1}^*{\bfE}_L({\bfE}_L^*{\bfE}_L)^{-1}{\bfE}_L^*\widehat{{\bfe}}_{k_1}\le\frac{u_0r}{n_1}=\frac{(n_cu_0)r}{n_cn_1}.
	\end{split}
	\end{equation*}
	\normalsize
%	where (a) holds due to (\ref{S_ps}).
	
	Similarly, we can prove $\left\|{\bfe}_{k_1}^*{{\bfU}}\right\|^2<\displaystyle
	\frac{(n_cu_0)r}{n_cn_1}$
	for all $i$ satisfying $1\le i\le n_cn_1$, which leads to \eqref{eqn:ratio}.
	\vspace{0.75mm}
	
	Moreover, we can provide a tighter bound on $\mu$ with a stronger assumption. Suppose there exists a $\widehat{d}\in\mathbb{C}$ and a real number $\delta\in (0,1)$ satisfying $(1-\delta)|\widehat{d}|\le |d_{k,i}| \le (1+\delta)|\widehat{d}|$. \\
	By {Lemma \ref{msp}}, define $\kappa_L=\frac{\sigma_{\max}({\bfE}_L)}{\sigma_{\min}({\bfE}_L)}$, then:
	\small
	\begin{equation*}
	\begin{split}
	&\lambda_{\max}({\bfD}_1^*{\bfE}_L^*{\bfE}_L{\bfD}_1)
	= \lambda_{\max}({\bfE}_L^*{\bfE}_L{\bfD}_1{\bfD}_1^*)\\
	&\le \lambda_{\max}({\bfE}_L^*{\bfE}_L)\lambda_{\max}({\bfD}_1{\bfD}_1^*)\\
	&\le \frac{\kappa_L^2(1+\delta)^2}{(1-\delta)^2} \lambda_{\min}({\bfE}_L^*{\bfE}_L)\lambda_{\min}({\bfD}_k{\bfD}_k^*)\\
	&\le \frac{\kappa_L^2(1+\delta)^2}{(1-\delta)^2} \lambda_{\min}({\bfD}_k^*{\bfE}_L^*{\bfE}_L{\bfD}_k).\\
	\end{split}
	\end{equation*}
	\normalsize
	since even the minimum eigenvalue of ${\bfD}_k^*{\bfE}_L^*{\bfE}_L{\bfD}_k$ is larger than the maximum one of $\frac{(1-\delta)^2}{\kappa_L^2(1+\delta)^2}{\bfD}_1^*{\bfE}_L^*{\bfE}_L{\bfD}_1$, we have
	$$\sum_{k=1}^{n_cn}{\bfD}_k^*{\bfE}_L^*{\bfE}_L{\bfD}_k\succeq [1+(n_c-1)\frac{(1-\delta)^2}{\kappa_L^2(1+\delta)^2}]{\bfD}_1^*{\bfE}_L^*{\bfE}_L{\bfD}_1.$$
	Similarly, we can establish the following relation between $\mu$ and $\mu_0$,
	\begin{equation*}
	\mu\le\frac{n_c\mu_0}{1+(n_c-1)\frac{(1-\delta)^2}{\kappa_L^2(1+\delta)^2}}.
	\end{equation*}
	%	When the frequencies of ${\bfX}$ are well separated\cite{liao2016music}, $\sigma_{\max}({\bfE}_L)$ and $\sigma_{\min}({\bfE}_L)$ are both proportional to $\sqrt{n_1}$. Therefore, when $n_c$ is large enough, $\mu\sim\mathcal{O}\Big((\frac{1+\delta}{1-\delta})^2\mu_0\Big)$.
\end{proof}

==> chapter_1/proof_publication_ready.tex <==
\vspace{-6mm}
\subsection{Supporting Lemmas for Theorem \ref{t1}}\label{t3l}
%The problem about convergence is reduced as showing the convergence of $\widetilde{\bfW}_{l}$. During each iteration, we claim that the distance between $\widetilde{{\bfW}}_{l}$ and $\mathcal{\widetilde{G}}{\bfY}$ decreases by a factor of $\nu<1$ in comparison with the last iteration. In the induction part, the proof is mainly based on properties of $\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}\widetilde{\mathcal{G}}{\mathcal{P}}_{\Omega}\widetilde{\mathcal{G}}^*\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}$. 

%\begin{theorem}\label{key_p}
%	Assume $0<\varepsilon_0<\frac{1}{10}$ and the following conditions\\
%	\begin{equation}\label{c1}
%	\left\|{\mathcal{P}}_{\Omega}\right\|\le 3\log(n),
%	\end{equation}
%	\begin{equation}\label{c2}
%	\left\|\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}\widetilde{\mathcal{G}}\widetilde{\mathcal{G}}^*\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}-p^{-1}\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}\widetilde{\mathcal{G}}{\mathcal{P}}_{\Omega}\widetilde{\mathcal{G}}^*\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}\right\|\le\varepsilon_0,
%	\end{equation}
%	\begin{equation}\label{c3}
%	\displaystyle\frac{\left\|\widetilde{{\bfL}}_0-\widetilde{\mathcal{G}}{\bfY}\right\|_F }{\sigma_{\min}(\widetilde{\mathcal{G}}{\bfY})}\le\displaystyle\frac{p^{1/2}\varepsilon_0}{6\log(n)(1+\varepsilon_0)}
%	\end{equation}
%	are satisfied. Then the iterate ${\bfY}_l$ in $(\ref{y_l})$ satisfies $\left\|{\bfY}_l-{\bfY}\right\|\le\nu^{l-1}\left\|\widetilde{{\bfL}}_0-\mathcal{\widetilde{G}}{\bfY}\right\|_F $ with $\nu =6\varepsilon_0<1$.
%\end{theorem}
%%The proof of {Theorem \ref{key_p}} can be found in \cite{CWW17}. Though we use different operators, the proof is only established on the properties of norm and structure of algorithm. We omit it since it is more important to verify the conditions in {Theorem \ref{key_p}}, especially (\ref{c2}), whose proof can be found in appendix. In general, the road map of the proofs follows closely with \cite{CWW17} as operator $\widetilde{\mathcal{G}}$ shares similar properties with operator $\mathcal{G}$. Hence, we omit some details in the following proof, which can be easily calculated according to \cite{CWW17}.\\

%In this section, some preliminary lemmas are presented. 
We first present some supporting lemmas to prove Theorem \ref{t1}. Lemma \ref{condition1} shows that the maximum number of repetitions is bounded by ${O}(\log n)$ with high probability in uniform sampling. {Lemma \ref{condition2}} derives the properties of $p^{-1}\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}\widetilde{\mathcal{G}}{\mathcal{P}}_{\Omega}\widetilde{\mathcal{G}}^*\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}$, and the random operator can be close enough to its mean $\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}\widetilde{\mathcal{G}}\widetilde{\mathcal{G}}^*\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}$ with a significant large amount of observed entries. {Lemma \ref{sub1}} connects the angle of two subspaces, represented as $\| \mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}-\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}}\|$, with $\|\widetilde{{\bfL}}_l-\widetilde{\mathcal{G}}{\bfY}\|_F$, and shows the angle decreases as $\bfL_l$ approaches to the ground truth. Lemma \ref{condition3} indicates the distance between the initial point and ground truth. {\black Lemmas \ref{condition2} and \ref{condition3} are built upon Lemmas 5 and 2 of \cite{CWW17}, respectively,  by extending   from single-channel signals to multi-channel signals.
 When $n_c=1$, Lemmas \ref{condition2} and \ref{condition3} are reduced to corresponding lemmas in \cite{CWW17}.}
%The proof of Lemma \ref{condition2} is similar to Lemma 3 in \cite{CC14} except some minor changes in the definitions of several operators, so the proof is skipped. 
\begin{lemma}
%	[\cite{R11}, Proposition 3.3]
	\label{condition1}
	Under sampling with replacement model, the maximum number of repetitions of any entry in $\Omega$ is less than $3\log(n)$ with probability at least $1-n_cn^{-2}$ for $n\ge 12$.
\end{lemma}
\begin{lemma}
	\label{condition2}
	Let $\widetilde{\mathcal{S}}$ be the tangent subspace of $\widetilde{\mathcal{H}}\bfX$. Assume $\mathcal{\widetilde{H}}{\bfX}$ is $\mu$-incoherent. Then with $m\ge32\mu c_sr\log(n)$,
%	Let $\widetilde{{\bfU}}\in C^{n_cn_1\times r}$ and $\widetilde{{\bfV}}\in C^{n_cn_2\times r}$ be two orthogonal matrices which satisfy
%	\begin{equation*}
%	\left\|\mathcal{P}_{\widetilde{{\bfU}}}(\widetilde{{\bfH}}_{k,t})\right\|_F^2\le \displaystyle\frac{\mu c_sr}{n_cn},\quad and\quad  \left\|\mathcal{P}_{\widetilde{{\bfV}}}(\widetilde{{\bfH}}_{k,t})\right\|_F^2\le \displaystyle\frac{\mu c_sr}{n_cn}.
%	\end{equation*}
%	Let ${\bf\mathcal{\widetilde{\mathcal{S}}}}$ be the subspace of $\widetilde{\mathcal{H}}\bfX$. Then with $m\ge32\mu c_sr\log(n)$,
	\begin{equation*}	
	\left\| \mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}}\widetilde{\mathcal{G}}\widetilde{\mathcal{G}}^*\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}}-p^{-1}\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}}\widetilde{\mathcal{G}}{\mathcal{P}}_{\Omega}\widetilde{\mathcal{G}}^*\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}} \right\|\le\displaystyle\sqrt{\frac{32\mu c_sr\log(n)}{m}}
	\end{equation*}
	holds with probability at least $1-n_cn^{-2}$.
\end{lemma}

\begin{lemma}[\cite{WCCL16}, Lemma 4.1]\label{sub1}
	Let ${\bfZ}_l$ be a rank-$r$ matrix and $\mathcal{S}_l$ be the tangent subspace of $\bfZ_l$. If $\bfZ$ is also a rank-$r$ matrix and its tangent subspace is denoted as $\mathcal{S}$, then 
	\begin{equation}\label{sub1.1}
	\left\| ({\mathcal{I}}-\mathcal{P}_{\mathcal{S}_l})(\bfZ_l-\bfZ) \right\|_F\le\displaystyle\frac{\left\|\bfZ_l-\bfZ\right\|_F^2 }{\sigma_{\rm min}(\bfZ)},\\
	\end{equation}
	\vspace{-2mm}
	\begin{equation}\label{sub1.3}
	\left\| \mathcal{P}_{\mathcal{S}_l}-\mathcal{P}_{\mathcal{S}}\right\|\le\displaystyle\frac{2\left\|\bfZ_l-\bfZ\right\|_F }{\sigma_{\rm min}(\bfZ)}.
	\end{equation}
\end{lemma}
\begin{lemma}\label{condition3}
	Assume $\mathcal{\widetilde{H}}{\bfX}$ is $\mu$-incoherent. With the initial point $\widetilde{{\bfL}}_0=\mathcal{Q}_r(p^{-1}\mathcal{\widetilde{H}}{\mathcal{P}}_{\Omega}({\bfX}))$, if $m\ge 16 \mu c_sr\log(n)$, we have
	\begin{equation*}
	\left\| \widetilde{{\bfL}}_0-\widetilde{\mathcal{H}}{\bfX} \right\|\le \displaystyle \sqrt{\frac{64\mu c_sr\log(n)}{m}}\left\| \widetilde{\mathcal{H}}{\bfX} \right\|
	\end{equation*} 
	holds with probability at least $1-n_cn^{-2}$.
\end{lemma}
%\input{proof_condition3.tex}

%\vspace{-10mm}
\subsection{Proof of Theorem \ref{t1}}\label{proof of 1}
{\black The proof of Theorem \ref{t1} is extended from  that of Theorem 3 in \cite{CWW17} with some modifications. %, while some parts are revised for the convenience of presentation in the proof of Theorem 2.  
The majority of the  efforts are devoted to the ``Inductive Step'' to build the connections between $\bfW_{l-1}$ and $\bfW_{l}$  through \eqref{I_4}. In \eqref{I_4}, the major issue is to bound %the four items, namely 
$I_1, I_2, I_3$ and $I_4$, and \eqref{eqn:t1.I124} and \eqref{eqn:t1.I3} provide critical steps in bounding these items. This inductive step is built upon a similar analysis for %One can find similar construction for
 $\bfL_l$'s in \cite{CWW17}. Here we study   $\bfW_{l}$'s instead of $\bfL_{l}$'s since the analysis of Theorem 2 is based on analyzing $\bfW_{l}$'s. 
 Although Lemma \ref{condition3} provides the theoretical bound for $\bfL_0$ directly,   a similar result for $\bfW_{0}$ is lacking. Thus, some efforts to analyze $\bfW_{0}$ is needed in the ``Base Case'' part. \eqref{eqn:m3} in Theorem \ref{t1} is obtained from  \eqref{eqn:t1.bound}, which provides the theoretical bound for the required number of observations to ensure successful recovery. We include detailed steps as follows for the completeness of the proof.}
%	 Finally, we add enough details for the completeness of the proof. }
\begin{proof}[Proof of Theorem \ref{t1}]
	As $\widetilde{{\bfL}}_{l+1}=\mathcal{Q}_r(\widetilde{{\bfW}_l})$, $\widetilde{{\bfL}}_{l+1}$ is the best rank-$r$ approximation to $\widetilde{{\bfW}}_l$. Then we have 
	\begin{equation}\label{W_L}
	\begin{split}
	\|\widetilde{{\bfL}}_{l+1}-\mathcal{\widetilde{G}}{\bfY}\|_F
	&\le \|\widetilde{{\bfW}}_l-\widetilde{{\bfL}}_{l+1}\|_F+\|\widetilde{{\bfW}}_{l}-\mathcal{\widetilde{G}}{\bfY}\|_F \\
	&\le 2\|\widetilde{{\bfW}}_{l}-\mathcal{\widetilde{G}}{\bfY}\|_F.
	\end{split}
	\end{equation}
	\normalsize
	Therefore, it is sufficient to bound $\|\widetilde{{\bfW}}_{l}-\mathcal{\widetilde{G}}{\bfY}\|_F$.
	{Lemma \ref{condition1}} suggests that with probability at least $1-n_cn^{-2}$, 
	\vspace{-1mm}
	\begin{equation}\label{c1}
	\|\mathcal{P}_{\Omega}\|\le 3\log(n)
	\vspace{-1mm}
	\end{equation}
	holds. 
	{Lemma \ref{condition2}} suggests as long as $m\ge 32\varepsilon_0^{-2}\mu c_sr\log(n)$,
	\vspace{-1mm}
	\begin{equation}\label{c2}
	\left\|\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}\widetilde{\mathcal{G}}\widetilde{\mathcal{G}}^*\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}-p^{-1}\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}\widetilde{\mathcal{G}}{\mathcal{P}}_{\Omega}\widetilde{\mathcal{G}}^*\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}\right\|\le\varepsilon_0
	\vspace{-1mm}
	\end{equation}  
	holds with probability at least $1-n_cn^{-2}$.
	
	Now we will show that the following inequality holds by mathematical induction, 
	\begin{equation}\label{c4}
	\displaystyle\frac{\|\widetilde{\bfW}_k-\widetilde{\mathcal{G}}{\bfY}\|_F }{\sigma_{\min}(\widetilde{\mathcal{G}}{\bfY})}\le\displaystyle\frac{p^{1/2}\varepsilon_0}{12\log(n)(1+\varepsilon_0)}.
	\end{equation}
	{\bf Inductive Step:} Suppose (\ref{c4}) holds for $k=l-1$. 
%	\begin{equation}\label{c4.1}
%	\displaystyle\frac{\left\|\widetilde{\bfW}_{l-1}-\widetilde{\mathcal{G}}{\bfY}\right\|_F }{\sigma_{\min}(\widetilde{\mathcal{G}}{\bfY})}\le\displaystyle\frac{p^{1/2}\varepsilon_0}{12\log(n)(1+\varepsilon_0)}.
%	\end{equation}
	Recall that
	\vspace{-2mm}
	\begin{equation*}
	\begin{split}
	\widetilde{{\bfW}}_l&=\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}\mathcal{\widetilde{H}}({\bfX}_l+p^{-1}\mathcal{P}_{\Omega}({\bfX}-{\bfX}_l))\\
	&=\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}\mathcal{\widetilde{G}}({\bfY}_l+p^{-1}\mathcal{P}_{\Omega}({\bfY}-{\bfY}_l)).
	\end{split}
	\vspace{-2mm}
	\end{equation*}
	Then, for all $ l\ge1$, we have
	\small
	\begin{equation*}
		\begin{split}
		&\left\|\widetilde{{\bfW}}_{l}-\mathcal{\widetilde{G}}{\bfY}\right\|_F
		=\left\|\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}\mathcal{\widetilde{G}}({\bfY}_l+p^{-1}\mathcal{P}_{\Omega}({\bfY}-{\bfY}_l)-\mathcal{\widetilde{G}}{\bfY}\right\|_F\\
		=& \left\|\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}\mathcal{\widetilde{G}}{\bfY}-\mathcal{\widetilde{G}}{\bfY}+(\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}\mathcal{\widetilde{G}}-p^{-1}\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}\mathcal{\widetilde{G}}\mathcal{P}_{\Omega})({\bfY}_l-{\bfY})\right\|_F\\
		\stackrel{(a)}{\le}&\left\|(\mathcal{I}-\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l})(\widetilde{{\bfL}}_l-\widetilde{\mathcal{G}}{\bfY})\right\|_F\\
		&+\left\|(\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}\mathcal{\widetilde{G}}\mathcal{\widetilde{G}}^*-p^{-1}\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}\mathcal{\widetilde{G}}\mathcal{P}_{\Omega}\mathcal{\widetilde{G}}^*)(\mathcal{P}_{\widetilde{\mathcal{S}}_l}\widetilde{{\bfW}}_{l-1}-\mathcal{\widetilde{G}}{\bfY})\right\|_F\\
		\le& \left\|(\mathcal{I}-\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l})(\widetilde{{\bfL}}_l-\widetilde{\mathcal{G}}{\bfY})\right\|_F+\left\|\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}\mathcal{\widetilde{G}}\mathcal{\widetilde{G}}^*(\mathcal{I}-\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l})(\widetilde{{\bfL}}_l-\widetilde{\mathcal{G}}{\bfY})\right\|_F\\
		&+\left\|(\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}\mathcal{\widetilde{G}}\mathcal{\widetilde{G}}^*\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}-p^{-1}\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}\mathcal{\widetilde{G}}\mathcal{P}_{\Omega}\mathcal{\widetilde{G}}^*\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l})(\widetilde{{\bfW}}_{l-1}-\mathcal{\widetilde{G}}{\bfY})\right\|_F\\
		&+p^{-1}\left\|\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}\mathcal{\widetilde{G}}\mathcal{P}_{\Omega}\mathcal{\widetilde{G}}^*(\mathcal{I}-\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l})(\widetilde{{\bfL}}_l-\widetilde{\mathcal{G}}{\bfY})\right\|_F\\
		\end{split}
		\end{equation*}
		\normalsize
		\vspace{-4mm}
		\begin{flalign}\label{I_4}
		& := I_1+I_2+I_3+I_4, &
		\end{flalign}		
	where (a) holds since $\widetilde{\bfL}_l=\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}\widetilde{\bfW}_{l-1}$.
	\normalsize
	By applying (\ref{sub1.1}),
	\begin{equation}\label{eqn:t1.I124}
	\begin{split}
	& I_1+I_2+I_4\\
	\le&\frac{2\|\widetilde{{\bfL}}_l-\mathcal{\widetilde{G}}{\bfY}\|_F^2 }{\sigma_{\min}(\mathcal{\widetilde{G}}{\bfY})}+p^{-1}\left\| \mathcal{P}_{\Omega}\mathcal{\widetilde{G}}^*\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}\right\|\frac{\|\widetilde{{\bfL}}_l-\mathcal{\widetilde{G}}{\bfY}\|_F^2 }{\sigma_{\min}(\mathcal{\widetilde{G}}{\bfY})} \\
	\le&\frac{8\|\widetilde{{\bfW}}_{l-1}-\mathcal{\widetilde{G}}{\bfY}\|_F^2 }{\sigma_{\min}(\mathcal{\widetilde{G}}{\bfY})}+4p^{-1}\left\| \mathcal{P}_{\Omega}\mathcal{\widetilde{G}}^*\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}\right\|\frac{\|\widetilde{{\bfW}}_{l-1}-\mathcal{\widetilde{G}}{\bfY}\|_F^2 }{\sigma_{\min}(\mathcal{\widetilde{G}}{\bfY})}.
	%&\le 2\varepsilon_0 \left\|\widetilde{{\bfL}}_l-\mathcal{\widetilde{G}}{\bfY}\right\|_F
	\end{split}
	\end{equation}
	Next, we will bound $\| \mathcal{P}_{\Omega}\mathcal{\widetilde{G}}^*\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}\|$. 
	For any ${\bfZ}\in \mathbb{C}^{n_cn_1\times n_cn_2}$, 
	\vspace{-1mm}
 	\begin{equation}
		\begin{split}
		\|\mathcal{P}_{\Omega}\widetilde{\mathcal{G}}^*\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}({\bfZ})\|^2
		=&\langle\mathcal{P}_{\Omega}\widetilde{\mathcal{G}}^*\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}({\bfZ}),\mathcal{P}_{\Omega}\widetilde{\mathcal{G}}^*\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}({\bfZ})\rangle		\\
		\stackrel{(b)}{\le}& 3\log(n)\langle\widetilde{\mathcal{G}}^*\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}({\bfZ}),\mathcal{P}_{\Omega}\widetilde{\mathcal{G}}^*\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}({\bfZ})\rangle\\
		=&3\log(n)\langle{\bfZ},\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}\widetilde{\mathcal{G}}\mathcal{P}_{\Omega}\widetilde{\mathcal{G}}^*\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}({\bfZ})\rangle\\
		\stackrel{(c)}{\le}& 3\log(n)(1+\varepsilon_0)p\left\|{\bfZ}\right\|_F^2.
		\end{split}
	\end{equation}
	\normalsize	
	where (b) holds due to (\ref{c1}), and (c) holds due to (\ref{c2}). Hence, $$\left\|\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}\widetilde{\mathcal{G}}\mathcal{P}_{\Omega}\right\|=\left\|\mathcal{P}_{\Omega}\widetilde{\mathcal{G}}^*\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}\right\|\le \sqrt{3\log(n)(1+\varepsilon_0)p},$$
	and
	\small
	\begin{equation}\label{sc1}
		\begin{split}
		&\left\|\mathcal{P}_{\Omega}\widetilde{\mathcal{G}}^*\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}\right\|\le\left\|\mathcal{P}_{\Omega}\widetilde{\mathcal{G}}^*(\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}-\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}})\right\|+\left\|\mathcal{P}_{\Omega}\widetilde{\mathcal{G}}^*\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}}\right\|\\
		\stackrel{(a)}{\le}& 3\log(n)\frac{2\|\widetilde{{\bfL}}_l-\mathcal{\widetilde{G}}{\bfY}\|_F }{\sigma_{\min}(\mathcal{\widetilde{G}}{\bfY})}+\left\|\mathcal{P}_{\Omega}\widetilde{\mathcal{G}}^*\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}}\right\|\\
		\stackrel{(b)}{\le}& 3\log(n)\frac{p^{1/2}\varepsilon_0}{3\log(n)(1+\varepsilon_0)}+\sqrt{3\log(n)(1+\varepsilon_0)p}\\
		\le& 3\log(n)(1+\varepsilon_0)p^{1/2},
		\end{split}
	\end{equation}
	\normalsize
	where (a) holds due to \eqref{sub1.3} and (\ref{c1}), and (b) holds due to (\ref{W_L}) and the inductive hypothesis.\\
	Hence, $I_1+I_2+I_4	\le 2\varepsilon_0 \|\widetilde{{\bfW}}_{l-1}-\mathcal{\widetilde{G}}{\bfY}\|_F$.
	Moreover, 
	\small
	\vspace{-1mm}
	\begin{align}\label{eqn:t1.I3}
		\begin{split}
		&\left\|\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}\widetilde{\mathcal{G}}\widetilde{\mathcal{G}}^*\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}-p^{-1}\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}\widetilde{\mathcal{G}}\mathcal{P}_{\Omega}\widetilde{\mathcal{G}}^*\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}\right\|\\
		\le&\left\|\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}}\widetilde{\mathcal{G}}\widetilde{\mathcal{G}}^*\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}}-p^{-1}\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}}\widetilde{\mathcal{G}}\mathcal{P}_{\Omega}\widetilde{\mathcal{G}}^*\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}}\right\|
		+\left\|(\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}-\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l})\widetilde{\mathcal{G}}\widetilde{\mathcal{G}}^*\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}\right\|\\
		&+\left\|\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}\widetilde{\mathcal{G}}\widetilde{\mathcal{G}}^*(\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}-\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l})\right\|+\left\|p^{-1}(\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}-\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l})\widetilde{\mathcal{G}}\mathcal{P}_{\Omega}\widetilde{\mathcal{G}}^*\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}\right\|\\
		&+\left\|p^{-1}\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}\mathcal{\widetilde{G}}\mathcal{P}_{\Omega}\widetilde{\mathcal{G}}^*(\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}-\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l})\right\|\\
%		\stackrel{(c)}{\le}&\varepsilon_0+\frac{4\|\widetilde{{\bfL}}_l-\widetilde{\mathcal{G}}{\bfY}\|_F}{\sigma_{\min}(\widetilde{\mathcal{G}}{\bfY})}\\
%		&+p^{-1}\frac{2\|\widetilde{{\bfL}}_l-\widetilde{\mathcal{G}}{\bfY}\|_F}{\sigma_{\min}(\widetilde{\mathcal{G}}{\bfY})}\Big(\left\|\mathcal{P}_{\Omega}\mathcal{\widetilde{G}}^*\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}\right\|+\left\|\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}\mathcal{\widetilde{G}}\mathcal{P}_{\Omega}\right\|\Big)\\
		\stackrel{(c)}{\le}&\varepsilon_0+\frac{2\|\widetilde{{\bfL}}_l-\widetilde{\mathcal{G}}{\bfY}\|_F}{\sigma_{\min}(\widetilde{\mathcal{G}}{\bfY})}\left(2+p^{-1}\|\mathcal{P}_{\Omega}\mathcal{\widetilde{G}}^*\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_l}\|+p^{-1}\|\mathcal{P}_\mathcal{\widetilde{\mathcal{S}}}\mathcal{\widetilde{G}}\mathcal{P}_{\Omega}\|   \right)\\
		\stackrel{(d)}{\le}& 4\varepsilon_0. 
		\end{split}
		\end{align}
		\normalsize
	where (c) comes from {Lemma \ref{sub1}}, and (d) comes from (\ref{c4}) and (\ref{sc1}). Then, $I_3$ can be bounded as
	\begin{equation}
	\vspace{-1mm}
	I_3\le 4\varepsilon_0\|\widetilde{{\bfW}}_{l-1}-\mathcal{\widetilde{G}}{\bfY}\|_F. 
	\end{equation}
	By putting pieces together, we have
	\begin{equation}\label{p_1}
	\|\widetilde{{\bfW}}_{l}-\mathcal{\widetilde{G}}{\bfY}\|_F\le\nu\|\widetilde{{\bfW}}_{l-1}-\mathcal{\widetilde{G}}{\bfY}\|_F.
	\end{equation} 
	Hence, (\ref{c4}) still holds for $k=l$.\\
	{\bf Base Case}: Let us assume
	\begin{equation}\label{initial}
	\|\widetilde{{\bfL}}_{0}-\mathcal{\widetilde{G}}{\bfY}\|_F\le\displaystyle\frac{p^{1/2}\varepsilon_0}{6\log(n)(1+\varepsilon_0)}.
	\end{equation}
	Then, similar to $I_1+I_2+I_3+I_4$ in \eqref{I_4}, we have
	\small
	\begin{equation*}
	\begin{split}
	&\left\|\widetilde{{\bfW}}_{0}-\mathcal{\widetilde{G}}{\bfY}\right\|_F
	=\left\|\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_0}\mathcal{\widetilde{G}}({\bfY}_0+p^{-1}\mathcal{P}_{\Omega}({\bfY}-{\bfY}_0))-\mathcal{\widetilde{G}}{\bfY}\right\|_F\\
%	\le& \left\|\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_0}\mathcal{\widetilde{G}}{\bfY}-\mathcal{\widetilde{G}}{\bfY}\right\|_F+\left\|(\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_0}\mathcal{\widetilde{G}}-p^{-1}\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_0}\mathcal{\widetilde{G}}\mathcal{P}_{\Omega})({\bfY}_0-{\bfY})\right\|_F\\
%	=&\left\|(\mathcal{I}-\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_0})(\widetilde{{\bfL}}_0-\widetilde{\mathcal{G}}{\bfY})\right\|_F\\
%	&+\left\|(\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_0}\mathcal{\widetilde{G}}\mathcal{\widetilde{G}}^*-p^{-1}\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_0}\mathcal{\widetilde{G}}\mathcal{P}_{\Omega}\mathcal{\widetilde{G}}^*)(\widetilde{{\bfL}}_0-\mathcal{\widetilde{G}}{\bfY})\right\|_F\\
	\le& \left\|(\mathcal{I}-\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_0})(\widetilde{{\bfL}}_0-\widetilde{\mathcal{G}}{\bfY})\right\|_F+\left\|\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_0}\mathcal{\widetilde{G}}\mathcal{\widetilde{G}}^*(\mathcal{I}-\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_0})(\widetilde{{\bfL}}_0-\widetilde{\mathcal{G}}{\bfY})\right\|_F\\
	&+\left\|(\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_0}\mathcal{\widetilde{G}}\mathcal{\widetilde{G}}^*\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_0}-p^{-1}\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_0}\mathcal{\widetilde{G}}\mathcal{P}_{\Omega}\mathcal{\widetilde{G}}^*\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_0})(\widetilde{{\bfL}}_0-\mathcal{\widetilde{G}}{\bfY})\right\|_F\\
	&+p^{-1}\left\|\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_0}\mathcal{\widetilde{G}}\mathcal{P}_{\Omega}\mathcal{\widetilde{G}}^*(\mathcal{I}-\mathcal{P}_{\mathcal{\widetilde{\mathcal{S}}}_0})(\widetilde{{\bfL}}_0-\widetilde{\mathcal{G}}{\bfY})\right\|_F\\
	\le& 5\varepsilon_0\|\widetilde{\bfL}_0-\widetilde{\mathcal{G}}\bfY\|_F.	
	\end{split}
	\end{equation*}
	\normalsize
	Since $\varepsilon_0\in (0, 1/10)$, we have
	\vspace{-3mm} $$\|\widetilde{{\bfW}}_{0}-\mathcal{\widetilde{G}}{\bfY}\|_F\le\frac{1}{2}\|\widetilde{{\bfL}}_{0}-\mathcal{\widetilde{G}}{\bfY}\|_F\le\displaystyle\frac{p^{1/2}\varepsilon_0}{12\log(n)(1+\varepsilon_0)},$$
    which completes the induction part.
    
    Then the only thing is to check the assumption (\ref{initial}). Using Lemma \ref{condition3} and  $\|\widetilde{{\bfL}}_0-\mathcal{\widetilde{G}}{\bfY}\|_F\le\sqrt{2r}\|\widetilde{{\bfL}}_0-\mathcal{\widetilde{G}}{\bfY}\|$, with probability at least $1-n_cn^{-2}$,
    \small
    \begin{equation*}
    \begin{split}
    \frac{\|\widetilde{{\bfL}}_0-\mathcal{\widetilde{G}}{\bfY}\|_F}{\sigma_{\min}(\mathcal{\widetilde{G}}{\bfY})}
    &\le\frac{\sqrt{2r}\|\widetilde{{\bfL}}_0-\mathcal{\widetilde{G}}{\bfY}\|}{\sigma_{\min}(\mathcal{\widetilde{G}}{\bfY})}
    =\kappa\sqrt{\frac{128\mu c_sr^2\log(n)}{m}}.
    \end{split}
    \end{equation*}
    \normalsize
    Therefore, to guarantee (\ref{initial}), we need
    \begin{equation}\label{eqn:t1.bound}
    \kappa\sqrt{\frac{128\mu c_sr^2\log(n)}{m}}\le \frac{p^{1/2}\varepsilon_0}{6\log(n)(1+\varepsilon_0)},
    \end{equation}
    That is  $m\ge C_1(1+\varepsilon_0)\varepsilon_0^{-1}n_c^{1/2}\mu^{1/2}c_s^{1/2}\kappa rn^{1/2}\log^{3/2}(n)$ with $C_1=48\sqrt{2}$.\\
    Hence, with probability at least $1-(2l+1)n_cn^{-2}$, from \eqref{p_1},
	\begin{equation}\label{eqn:t1.linear_convergence}
	\begin{split}
	\left\|{\bfY}_l-{\bfY}\right\|_F 
	&=\|\mathcal{\widetilde{G}}^*(\widetilde{{\bfL}}_l-\mathcal{\widetilde{G}}{\bfY})\|_F
	\le\|\widetilde{{\bfL}}_l-\mathcal{\widetilde{G}}{\bfY}\|_F\\
	&\le2\|\widetilde{{\bfW}}_{l-1}-\mathcal{\widetilde{G}}{\bfY}\|_F\le2\nu^{l-1}
	\|\widetilde{{\bfW}}_0-\mathcal{\widetilde{G}}{\bfY}\|_F \\
	&\le \nu^{l-1}
	\|\widetilde{{\bfL}}_0-\mathcal{\widetilde{G}}{\bfY}\|_F,
	\end{split} 
	\end{equation}
	where ${\bfY}_l=\widetilde{\mathcal{G}}^*\widetilde{{\bfL}}_l,\mathcal{\widetilde{G}}^*\mathcal{\widetilde{G}}=\mathcal{I}$ and $\|\mathcal{\widetilde{G}}^*\|\le 1$.
\end{proof}
\subsection{Proof of Theorem \ref{t4}}
First, we extend the eigenvalues and eigenvectors of linear operators on vector spaces to the eigenvalues and eigenmatrices of linear operators on matrix spaces, defined as follows. 
\begin{defi} \label{defi: eigenmatrix}
	Let $\mathcal{A}$ denote a linear operator from $\mathbb{C}^{l_1\times l_2}$ to $\mathbb{C}^{l_1\times l_2}$,
	for any matrix $\bfM$ in the space and $\bfM\neq \mathbf{0}$, if $\mathcal{A}\bfM=\lambda \bfM$ holds, then $\bfM$ is one eigenmatrix of operator $\mathcal{A}$, and $\lambda$ is the corresponding eigenvalue. 
\end{defi}
Let $\mathcal{L}$ denote the following linear operator on the matrix space $\mathbb{C}^{n_cn_1\times n_cn_2}$, $$\mathcal{L}=\mathcal{P}_{\widetilde{\mathcal{S}}}\widetilde{\mathcal{G}}\widetilde{\mathcal{G}}^*\mathcal{P}_{\widetilde{\mathcal{S}}}-p^{-1}\mathcal{P}_{\widetilde{\mathcal{S}}}\widetilde{\mathcal{G}}\mathcal{P}_\Omega\widetilde{\mathcal{G}}^*\mathcal{P}_{\widetilde{\mathcal{S}}}.$$ 
We first introduce Lemmas \ref{lemma: linear approximation of update rule}, \ref{lemma: real eigenvalues} and \ref{lemma: convergence rate with eigenvalue} that are useful in the proof of Theorem \ref{t4}. % mainly analyze the eigenvalues of $\mathcal{L}$. The proof of Theorem \ref{t4} is established on the three lemmas.

\begin{lemma}\label{lemma: linear approximation of update rule}
Suppose that for any  $\epsilon>0$,  there always exists an integer $s_\epsilon$ such that for any integer $k\geq 0$,  the iterates $\widetilde{\bfW}_{s_\epsilon+k}$ generated by AM-FIHT satisfy $\|\widetilde{\bfW}_{s_\epsilon+k}-\widetilde{\mathcal{G}}\bfY\|_F\leq \epsilon$. Then	with any $l>s_\epsilon+1$, the updated rule can be denoted as
	{	\footnotesize
	\begin{equation*}
	\begin{split}
	& \begin{bmatrix}
	\widetilde{\bfW}_l-\widetilde{\mathcal{G}}{\bfY}\\
	\widetilde{\bfW}_{l-1}-\widetilde{\mathcal{G}}{\bfY}
	\end{bmatrix}
	= \begin{bmatrix}
	\mathcal{L}(\widetilde{\bfW}_{l-1}-\widetilde{\mathcal{G}}{\bfY}) +\beta \mathcal{P}_{\widetilde{\mathcal{S}}} (\widetilde{\bfW}_{l-1}-\widetilde{\bfW}_{l-2})\\
	\widetilde{\bfW}_{l-1}-\widetilde{\mathcal{G}}{\bfY} 
	\end{bmatrix}+\widetilde{\bfZ}_{l-1},
	\end{split}
	\end{equation*}
	\normalsize
	where 
	\small
	\begin{equation*}
	\left\|\widetilde{\bfZ}_{l-1}\right\|_F=o\left(
	\left\|
	\begin{bmatrix}
	\widetilde{\bfW}_{l-1}-\widetilde{\mathcal{G}}{\bfY}\\
	\widetilde{\bfW}_{l-2}-\widetilde{\mathcal{G}}{\bfY}
	\end{bmatrix}
	\right\|_F
	\right).
	\end{equation*}}
	\normalsize
%	$$\widetilde{\bfW}_l=\widetilde{\mathcal{G}}{\bfY}+\mathcal{L}(\widetilde{\bfW}_{l-1}-\widetilde{\mathcal{G}}{\bfY})+{\bfZ}_{l-1},$$
	%	where $\left\|{\bfZ}_{l-1}\right\|_F=o(\|\widetilde{\bfW}_{l-1}-\widetilde{\mathcal{G}}{\bfY}\|_F)$.
	%	and $\mathcal{L}=\mathcal{P}_{\widetilde{\mathcal{S}}}\widetilde{\mathcal{G}}\widetilde{\mathcal{G}}^*\mathcal{P}_{\widetilde{\mathcal{S}}}-p^{-1}\mathcal{P}_{\widetilde{\mathcal{S}}}\widetilde{\mathcal{G}}\mathcal{P}_\Omega\widetilde{\mathcal{G}}^*\mathcal{P}_{\widetilde{\mathcal{S}}} $.
\end{lemma}
%\input{proof_update.tex}

\begin{lemma}\label{lemma: real eigenvalues}
	All the eigenvalues of operator $\mathcal{L}$
	are real numbers.
\end{lemma}
%\input{proof_eig.tex}
\begin{lemma}[\cite{P87}, Lemma 2.1]\label{lemma: convergence rate with eigenvalue}
	Let $\mathcal{A}$ be a linear operator from $\mathbb{C}^{l_1\times l_2}$ to $\mathbb{C}^{l_1\times l_2}$, and let $\lambda_1,\cdots,\lambda_n$ be its eigenvalues, let $\rho(\mathcal{A})=\max_{1\leq i\leq n}|\lambda_i|$, if $\rho(\mathcal{A})<1$, then there exists some constant $c(\delta)$ such that $\|\mathcal{A}^k\|\leq c(\delta)(\rho(\mathcal{A})+\delta)^k$ holds for all integers $k$, where $0< \delta<1-\rho(\mathcal{A}).$
\end{lemma}

%\begin{proof} 
%	Lemma \ref{lemma: convergence rate with eigenvalue} is the extension of lemma 1 in chapter 2 of \cite{P87} to the linear operators on matrix spaces. Based on the following property
%	\begin{equation*}
%		\rho(\mathcal{A})=\lim_{k\rightarrow \infty}\|\mathcal{A}^k\|^{1/k}<1,
%	\end{equation*}
%	we can bound
%	the spectral norm of $\mathcal{A}^k$ as 
%	\begin{equation*}
%		\|\mathcal{A}^k\|\leq c(\rho(\mathcal{A})+\delta)^k,
%	\end{equation*}
%	where $0<\delta<1-\rho(\mathcal{A}), c$ is a constant. Therefore, 
%	\small
%	\begin{equation*}
%		\begin{split}
%			\|\mathcal{A}^k(\bfZ)\|_F & \leq \|\mathcal{A}^k\|\|\bfZ\|_F \leq c(\rho(\mathcal{A})+\delta)^k \epsilon=c(\epsilon)(\rho(\mathcal{A})+\delta)^k.
%		\end{split}
%	\end{equation*}
%	\normalsize
%\end{proof}
\begin{proof}[Proof of Theorem \ref{t4}]	
	First, we claim that AM-FIHT is still convergent with a small $\beta\in (0,1).$
	Based on the proof of Theorem \ref{t1}, 
	\vspace{-1mm}
	$$\| \widetilde{\bfW}_l-\widetilde{\mathcal{G}}{\bfY}\| _F\leq \nu \| \widetilde{\bfW}_{l-1}-\widetilde{\mathcal{G}}{\bfY}\| _F,$$ 
	\normalsize
	where $\nu=6\varepsilon_0, 0<\varepsilon_0< {1}/{10}$. 	
	A loose bound from a direct derivation with $\beta\neq 0$ is 
	\begin{equation*}
	\|\widetilde{\bfW}_l-\widetilde{\mathcal{G}}{\bfY}\|_F\leq (\nu+\beta) \|\widetilde{\bfW}_{l-1}-\widetilde{\mathcal{G}}{\bfY}\|_F+\beta\|\widetilde{\bfW}_{l-2}-\widetilde{\mathcal{G}}{\bfY}\|_F. 
	\end{equation*}
	\normalsize
	Thus if $\nu+2\beta<1,$ i.e., $\beta\in(0,\frac{1}{5}),$ the iteration is still convergent. Thus for any $\epsilon>0$, we can always find such an $l$ that $\|\widetilde{\bfW}_{l-2+k}-\widetilde{\mathcal{G}}\bfY\|_F\leq \epsilon, \forall k\geq0.$
	%However, this only serves as an extremely loose bound. To achieve the tight one, we need some additional Lemmas for preparations. Recall the definition of eigendecomposition, the eigenmatrices and eigenvalues of linear operators is defined as the extension of matrix eigenvectors and eigenvalues: $\bfM$ and $\lambda$ are one eigenmatrix and the corresponding eigenvalue of a linear operator $\mathcal{F}$, if $\mathcal{F}(\bfM)=\lambda \bfM$. Let $\mathcal{L}$ denote the linear operator $\mathcal{P}_{\widetilde{\mathcal{S}}}\widetilde{\mathcal{G}}\widetilde{\mathcal{G}}^*\mathcal{P}_{\widetilde{\mathcal{S}}}-p^{-1}\mathcal{P}_{\widetilde{\mathcal{S}}}\widetilde{\mathcal{G}}\mathcal{P}_\Omega\widetilde{\mathcal{G}}^*\mathcal{P}_{\widetilde{\mathcal{S}}}$, 
	Then following {Lemma \ref{lemma: linear approximation of update rule}}, 
	%	we have
	%	\begin{equation*}
	%	\begin{split}
	%	\mathcal{P}_{\widetilde{\mathcal{S}}}(\widetilde{\bfW}_l)&
	%	=\mathcal{P}_{\widetilde{\mathcal{S}}}(\widetilde{\mathcal{G}}{\bfY})+\mathcal{P}_{\widetilde{\mathcal{S}}}\mathcal{L}(\widetilde{\bfW}_{l-1}-\widetilde{\mathcal{G}}{\bfY})+\mathcal{P}_{\widetilde{\mathcal{S}}}({\bfZ}_{l-1})\\
	%	&=\widetilde{\mathcal{G}}{\bfY}+\mathcal{L}(\widetilde{\bfW}_{l-1}-\widetilde{\mathcal{G}}{\bfY})+\mathcal{P}_{\widetilde{\mathcal{S}}}({\bfZ}_{l-1}).
	%	\end{split}
	%	\end{equation*}
	if we ignore $\widetilde{\bfZ}_{l-1}$,
	%	then $\mathcal{P}_{\widetilde{\mathcal{S}}}(\widetilde{\bfW}_l)=\widetilde{\bfW}_l$. With $\beta\neq 0,$ we have
	%	\begin{equation*}
	%	\begin{split}
	%	\widetilde{\bfW}_l&-\widetilde{\mathcal{G}}{\bfY}
	%	=\mathcal{L}(\widetilde{\bfW}_{l-1}-\widetilde{\mathcal{G}}{\bfY})+\beta\mathcal{P}_{\widetilde{\mathcal{S}}}(\widetilde{\bfW}_{l-1}-\widetilde{\bfW}_{l-2})\\
	%	=&\mathcal{L}(\widetilde{\bfW}_{l-1}-\widetilde{\mathcal{G}}{\bfY})+\beta(\widetilde{\bfW}_{l-1}-\widetilde{\mathcal{G}}{\bfY})-\beta(\widetilde{\bfW}_{l-2}-\widetilde{\mathcal{G}}{\bfY}).
	%	\end{split}
	%	\end{equation*}
	then 
	\begin{equation*}
	\widetilde{\bfW}_l-\widetilde{\mathcal{G}}{\bfY}=\mathcal{L}(\widetilde{\bfW}_{l-1}-\widetilde{\mathcal{G}}{\bfY}) +\beta \mathcal{P}_{\widetilde{\mathcal{S}}} (\widetilde{\bfW}_{l-1}-\widetilde{\bfW}_{l-2}).
	\end{equation*}
	Thus $\mathcal{P}_{\widetilde{\mathcal{S}}}(\widetilde{\bfW}_l-\widetilde{\mathcal{G}}{\bfY})=\widetilde{\bfW}_l-\widetilde{\mathcal{G}}{\bfY}$.
	With $\mathcal{P}_{\widetilde{\mathcal{S}}}(\widetilde{\mathcal{G}}{\bfY})=\widetilde{\mathcal{G}}{\bfY},$ we have $\mathcal{P}_{\widetilde{\mathcal{S}}}(\widetilde{\bfW}_l)=\widetilde{\bfW}_l.$
	% \begin{equation*}
	% \mathcal{P}_{\widetilde{\mathcal{S}}}(\widetilde{\bfW}_l-\widetilde{\mathcal{G}}{\bfY})=\widetilde{\bfW}_l-\widetilde{\mathcal{G}}{\bfY}.
	% \end{equation*}
	The update rule of AM-FIHT can be further simplified as 
	\small
	\begin{equation*}
	\begin{split}
	\begin{bmatrix}
	\widetilde{\bfW}_l-\widetilde{\mathcal{G}}{\bfY}\\
	\widetilde{\bfW}_{l-1}-\widetilde{\mathcal{G}}{\bfY}
	\end{bmatrix}
	=& \begin{bmatrix}
	\mathcal{L}(\widetilde{\bfW}_{l-1}-\widetilde{\mathcal{G}}{\bfY}) +\beta(\widetilde{\bfW}_{l-1}-\widetilde{\bfW}_{l-2})\\
	\widetilde{\bfW}_{l-1}-\widetilde{\mathcal{G}}{\bfY} 
	\end{bmatrix}\\
	:=&
	\widetilde{\mathcal{L}}\begin{bmatrix}
	\widetilde{\bfW}_{l-1}-\widetilde{\mathcal{G}}{\bfY}\\
	\widetilde{\bfW}_{l-2}-\widetilde{\mathcal{G}}{\bfY}
	\end{bmatrix}.
	\end{split}
	\end{equation*}
	\normalsize
	Following Lemma \ref{condition2}, we have  $\left\|\mathcal{L} \right\|<1$, if $m>32\mu c_sr\log(n)$. Based on the definitions of $\rho(\mathcal{L})$ and $\|\mathcal{L}\|$, we have $\rho(\mathcal{L})\leq \|\mathcal{L}\|<1$.
	Our aim is to prove $\rho(\widetilde{\mathcal{L}})<\rho(\mathcal{L})$. 
	%	Since $\rho(\widetilde{\mathcal{L}})$ is determined by nonzero eigenvalues, here we only consider the nonzero ones. 
	Let $\lambda$ denote one nonzero eigenvalue of $\widetilde{\mathcal{L}}$, the corresponding eigenmatrix is 
	$
	\begin{bmatrix}
	\bfM_1\\
	\bfM_2
	\end{bmatrix}
	$, then
	\begin{equation*}
	\widetilde{\mathcal{L}}
	\begin{bmatrix}
	{\bfM}_1\\
	{\bfM}_2\\
	\end{bmatrix}
	=\begin{bmatrix}
	\mathcal{L}\bfM_1 +\beta (\bfM_1-\bfM_2)\\
	\bfM_1 	\end{bmatrix}
	=\lambda 
	\begin{bmatrix}
	{\bfM}_1\\
	{\bfM}_2\\
	\end{bmatrix},
	\end{equation*}
	\normalsize
	we have ${\bfM}_1=\lambda {\bfM}_2, \mathcal{L}({\bfM}_1)+\beta {\bfM}_1-\beta {\bfM}_2=\lambda {\bfM}_1$.  Therefore, $\lambda \mathcal{L}({\bfM}_2)+\lambda \beta {\bfM}_2-\beta {\bfM}_2=\lambda^2 {\bfM}_2$. With $\lambda\neq 0$, 
	\begin{equation*}
	\mathcal{L}(\bfM_2)=(\lambda-\beta+\beta/\lambda)\bfM_2 :=\eta_i \bfM_2,
	\end{equation*}
	thus ${\bfM}_2$ is an eigenmatrix of operator $\mathcal{L},$ with the corresponding eigenvalue as $\eta_i$. Lemma \ref{lemma: real eigenvalues} shows $\eta_i\in \mathbb{R}$, then we have
	\begin{equation*}
	\lambda^2-\eta_i \lambda-\beta \lambda+\beta=0,
	\end{equation*}
	\begin{equation*}
	\begin{split}
	& \lambda_{i1}=\frac{\eta_i+\beta+ \sqrt{(\eta_i+\beta)^2-4\beta}}{2},\\
	& \lambda_{i2}=\frac{\eta_i+\beta- \sqrt{(\eta_i+\beta)^2-4\beta}}{2}.
	\end{split}
	\end{equation*}
	Here we analyze in two cases:
	\begin{enumerate}
		\item for any $\eta_i$ that satisfies $(\eta_i+\beta)^2-4\beta\leq 0$, the modulus $|\lambda_{i1}|=|\lambda_{i2}|=\sqrt{\beta}$. 
		\item for any $\eta_i$ that satisfies $(\eta_i+\beta)^2-4\beta>0,\eta_i$ cannot be zero for any $\beta\in(0,1)$.   
		 With $\rho(\mathcal{L})=\max_i |\eta_i|<1$, it holds that $\eta_i<1$. In this case, with $\beta\in (0,1)$, we have
		\begin{equation*}
		\begin{split}
		(\eta_i+\beta)^2-4\beta =(\eta_i-\beta)^2-4(1-\eta_i)\beta<(\eta_i-\beta)^2,
		\end{split}
		\end{equation*}
%		Thus, 
		\begin{equation*}
		\begin{split}
		&  \max\{|\lambda_{i1}|,|\lambda_{i2}|\}= \frac{|\eta_i+\beta|+ \sqrt{(\eta_i+\beta)^2-4\beta}}{2}\\
		&< \frac{|\eta_i+\beta|+|\eta_i-\beta|}{2} = \max\{|\eta_i|, \beta\} \leq \max\{|\eta_i|, \sqrt{\beta}\}.
		\end{split}
		\end{equation*}
	\end{enumerate}
	Combining the two cases, if we choose a positive $\beta$ that satisfies $\beta<\left(\max_i\{|\eta_i|\}\right)^2=\rho^2(\mathcal{L})$, let
	\begin{equation}\label{eqn: expression of q}
	q(0)=\rho(\mathcal{L}), q(\beta)=\rho(\widetilde{\mathcal{L}}), \tau= \min\left\{1/5, \rho^2(\mathcal{L})\right\},
	\end{equation}
	then we have $q(0)>q(\beta), \forall \beta\in (0,\tau).$
\end{proof}

%	\begin{equation*}
%	\begin{split}
%	0<(\eta_i+\beta)^2-4\beta =& (\eta_i-\beta)^2-4(1-\eta_i)\beta\\
%	<& \left(|\eta_i-\beta|-\frac{2(1-\eta_i)\beta}{|\eta_i-\beta|}\right)^2,
%	\end{split}
%	\end{equation*}
%	\begin{equation*}
%	\frac{(1-\eta_i)\beta}{|\eta_i-\beta|}\geq \frac{(1-\max_i|\eta_i|)\beta}{\max_i|\eta_i|+\beta}=\frac{(1-\rho(\mathcal{L}))\beta}{\rho(\mathcal{L})+\beta}>0,
%	\end{equation*}
%	if we set $\beta$ satisfying 
%	\begin{equation*}
%	|\eta_i-\beta|-\frac{2(1-\eta_i)\beta}{|\eta_i-\beta|}\geq 0, \ \forall \eta_i\neq 0,
%	\end{equation*}
%	$\text{i.e.}, \beta\leq1-\sqrt{1-\eta_i^2}$ holds, $\forall \eta_i\neq 0$, then
%	\small
%	\begin{equation*}
%		\begin{split}
%		& \max\{|\lambda_{i1}|,|\lambda_{i1}|\} = \frac{|\eta_i+\beta|+ \sqrt{(\eta_i+\beta)^2-4\beta}}{2}\\
%		 <& \frac{1}{2}\left(|\eta_i+\beta|+|\eta_i-\beta|-\frac{2\beta(1-\rho(\mathcal{L}))}{\rho(\mathcal{L})+\beta}\right)\\
%		=& \max\{|\eta_i|, \beta\}-\frac{\beta(1-\rho(\mathcal{L}))}{\rho(\mathcal{L})+\beta}.
%		\end{split}
%		\end{equation*}
%		\normalsize
%\end{enumerate}
%Thus if $\beta$ is small enough such that  $\sqrt{\beta}\leq \rho(\mathcal{L})-\frac{\beta(1-\rho(\mathcal{L}))}{\rho(\mathcal{L})+\beta}$ also holds, then we have
%\vspace{-2mm}
%\begin{equation*}
%\vspace{-2mm}
%\rho(\widetilde{\mathcal{L}})<\rho(\mathcal{L})-\frac{\beta(1-\rho(\mathcal{L}))}{\rho(\mathcal{L})+\beta}.
%\end{equation*}
%Let 
%\vspace{-1mm}
%\begin{equation}\label{eqn: expression of q}
%\vspace{-1mm}
%q(0)=\rho(\mathcal{L}),\quad q(\beta)=\rho(\widetilde{\mathcal{L}}),
%\end{equation}
% from Lemma \ref{lemma: convergence rate with eigenvalue}, Theorem \ref{t4} holds. 
%\end{proof}

\subsection{Proof of Theorem \ref{t2}}\label{proof of 2}
Lemma \ref{t2c1} derives the properties of {\small$\widehat{p}^{-1}\mathcal{P}_{\widehat{\mathcal{S}}_l}\widetilde{\mathcal{G}}{\mathcal{P}}_{\Omega_{l+1}}\widetilde{\mathcal{G}}^*(\mathcal{{P}}_{\widetilde{{\bfU}}}-\mathcal{{P}}_{\widehat{{\bfU}}_l})$}, and the random operator can be close enough to its mean {\small $\mathcal{P}_{\widehat{\mathcal{S}}_l}\widetilde{\mathcal{G}}\widetilde{\mathcal{G}}^*(\mathcal{{P}}_{\widetilde{{\bfU}}}-\mathcal{{P}}_{\widehat{{\bfU}}_l})$} with a significant large amount of observed entries. Lemma \ref{t2c2} illustrates the relation between $\widetilde{\bfL}_l$ and $\widetilde{\bfL}^{\prime}_l$ and gives the bound on the incoherence of $\widetilde{\bfL}^{\prime}_l$, which is obtained after the trimming part (line $5$ to $10$). {\black  Lemmas \ref{t2c1} and \ref{t2c2} are built upon Lemmas 9 and 10 in \cite{CWW17} by extending from single-channel signals to multi-channel signals. Similar to the proof of Theorem 1, the proof of Theorem 3 is built upon that of Lemma 3 in \cite{CWW17}, which is originally proposed as an initialization strategy. The major steps are devoted to bounding $I_5, I_6$ and $I_7$ in \eqref{I_567}, and the corresponding results are presented in \eqref{eqn:I_5}, \eqref{eqn:I_6}, and \eqref{eqn:I_7}. We include some details for the completeness of this proof. 
}
%With minor change in several operators, the proof of Lemma \ref{t2c1} is similar to that of Lemma 9 in \cite{CWW17}. The proof of Lemma \ref{t2c2} follows the major step in the proof of Lemma 4.10 in \cite{WCCL16}. Though different operators are used in these two lemmas, the corresponding operators in these two lemmas share critical properties. The proofs of Lemmas \ref{t2c1} and \ref{t2c2} are skipped.
%The proof of Lemma \ref{t2c1} can be directly derived from the proof of {Lemma \ref{condition2}}, or it will be also clear from a similar lemma for single channel Hankel operator that proposed in \cite{CWW17}. Additionally, since the proof of {Lemma \ref{t2c2}} mainly depends on derivation of $\bfA_l$ and $\bfB_l$, one can find the proof in . 

\begin{lemma}\label{t2c1}
	Let  $\widetilde{{\bfL}}^{\prime}_l=\widehat{{\bfU}}_l\widehat{{\bf\Sigma}}_l\widehat{{\bfV}}_l^*$ and $\widetilde{\mathcal{G}}\bfY=\widetilde{{\bfU}}\widetilde{{\bf\Sigma}}\widetilde{{\bfV}}^*$ be the SVD of $\widetilde{{\bfL}}_l^{\prime}$ and $\widetilde{\mathcal{G}}\bfY$. Further let $\widehat{\mathcal{S}}_l$ be the tangent subspace of $\widetilde{{\bfL}}^{\prime}_l$. Assume there exists a constant $\mu$ such that
	\vspace{-2mm}
	\begin{equation*}
	\vspace{-1mm}
	\left\| \mathcal{P}_{\widehat{{\bfU}}_l}\widetilde{{\bfH}}_{k,t}\right\|_F^2\le \frac{\mu c_sr}{n_cn}, \quad \left\| \mathcal{P}_{\widehat{{\bfV}}_l}\widetilde{{\bfH}}_{k,t}\right\|_F^2\le \frac{\mu c_sr}{n_cn},
	\end{equation*}
	and
	\vspace{-1mm}
	\begin{equation*}
	\left\| \mathcal{P}_{\widetilde{{\bfU}}}\widetilde{{\bfH}}_{k,t}\right\|_F^2\le \frac{\mu c_sr}{n_cn}, \quad \left\| \mathcal{P}_{\widetilde{{\bfV}}}\widetilde{{\bfH}}_{k,t}\right\|_F^2\le \frac{\mu c_sr}{n_cn}.
	\end{equation*}
	for all $1\le t \le n, 1\le k \le n_c$. Let $\Omega_{l+1}=\{(k_a,t_a)|a=1,\cdots,\widehat{m}\}$ be a set of indices sampled with replacement. If ${\mathcal{P}}_{\Omega_{l+1}}$ is independent of $\widetilde{{\bfU}}$, $\widetilde{{\bfV}}$, $\widehat{{\bfU}}_l$ and $\widehat{{\bfV}}_l$, then
	\vspace{-2mm}
	\begin{equation*}
	\left\|\mathcal{P}_{\widehat{\mathcal{S}}_l}\widetilde{\mathcal{G}}({\mathcal{I}}-\widehat{p}^{-1}{\mathcal{P}}_{\Omega_{l+1}})\widetilde{\mathcal{G}}^*(\mathcal{{P}}_{\widetilde{{\bfU}}}-\mathcal{{P}}_{\widehat{{\bfU}}_l})\right\|\le \sqrt{\frac{160\mu c_s r \log(n)}{\widehat{m}}}
	\end{equation*}
	with probability at least $1-n_cn^{-2}$, if $\widehat{m}\ge\frac{125}{18}\mu c_s r \log(n)$.
\end{lemma} 
\begin{lemma}\label{t2c2}
	Let $\widetilde{{\bfL}}_l=\widetilde{{\bfU}}_l\widetilde{{\bf\Sigma}}_l\widetilde{{\bfV}}_l^*$ and $\widetilde{\mathcal{G}}{\bfY}=\widetilde{{\bfU}}\widetilde{{\bf\Sigma}}\widetilde{{\bfV}}^*$ be the SVD of $\widetilde{{\bfL}}_l$ and $\widetilde{\mathcal{G}}\bfY$. Assume 
	$$\max_{k_1}||\widetilde{{\bfU}}_{k_1*}||^2\le \frac{\mu c_s r}{n_cn} \  \text{and}\  \max_{k_2}||\widetilde{{\bfV}}_{k_2*}||^2\le 
	\frac{\mu c_s r}{n_cn}.$$	
	Suppose $\widetilde{{\bfL}}_l$ and $\widetilde{\mathcal{G}}{\bfY}$ are both rank-$r$ matrices satisfying
	\vspace{-2mm}
	\begin{equation*}
	\vspace{-1mm}
	\|\widetilde{{\bfL}}_l-\widetilde{\mathcal{G}}{\bfY}\|_F\le\frac{\sigma_{\min}(\widetilde{\mathcal{G}}{\bfY})}{10\sqrt{2}}. 
	\end{equation*}
%	Assume $||\widetilde{{\bfU}}_{k_1*}||^2\le \frac{\mu c_s r}{n_cn}, \forall k_1$ and $||\widetilde{{\bfV}}_{k_2*}||^2\le 
%	\frac{\mu c_s r}{n_cn}, \forall k_2$. 
	Then the matrix $\widetilde{{\bfL}}^{\prime}_l=\widehat{{\bfU}}_l\widehat{{\bf\Sigma}}_l\widehat{{\bfV}}_l^*$, denoting the SVD of $\widetilde{{\bfL}}_l^{\prime}$, that is obtained after trimming in RAM-FIHT satisfies 
	\vspace{-1mm}
	\begin{equation}\label{eqn: t2c2_1}
	\begin{split}
	\| \widetilde{{\bfL}}^{\prime}-\widetilde{\mathcal{G}}{\bfY}\|_F\le 8\kappa\|\widetilde{{\bfL}}_l-\widetilde{\mathcal{G}}{\bfY}\|_F,   
	\end{split} 
	\end{equation}
	\begin{equation}\label{eqn: t2c2_2}
	\max_{k_1,k_2}\bigg\{\|\widehat{{\bfU}}_{k_1*}\|^2,\|\widehat{{\bfV}}_{k_2*} \|^2  \bigg\}\le\frac{100\mu c_s r}{81n_cn},  
	\end{equation}
	\normalsize
	where $\kappa$ denotes the condition number of $\widetilde{\mathcal{G}}{\bfY}$.
\end{lemma}


\begin{proof}[Proof of Theorem \ref{t2}]
	First, we show the following inequality holds with high probability by mathematical induction.
	\begin{equation}\label{3.1}
	\|\widetilde{{\bfL}}_k-\widetilde{\mathcal{G}}{\bfY}\|_F\le\frac{\varepsilon_0\sigma_{\min}(\widetilde{\mathcal{G}}{\bfY})}{128\kappa^2}. 
	\end{equation}
	{\bf Inductive Step:} Suppose (\ref{3.1}) holds when $k=l$ and $l\ge0$. Then \eqref{eqn: t2c2_2} in Lemma \ref{t2c2} holds.  
%	By {Lemma \ref{t2c2}}, we have
%	\begin{equation}\label{3.2}
%	\begin{split}
%	\left\|\widetilde{{\bfL}}^{\prime}_l-\widetilde{\mathcal{G}}{\bfY} \right\|_F\le 8\kappa \left\|\widetilde{{\bfL}}_l-\widetilde{\mathcal{G}}{\bfY} \right\|_F \quad \text{and} \quad\\ \max\Bigg\{\left\|\widehat{{\bfU}}^{(k_1,:)}\right\|^2, \left\| \widehat{{\bfV}}^{(k_2,:)}\right\|^2  \Bigg\} \le \frac{100\mu c_s r}{81n_cn} 
%	\end{split}
%	\end{equation}
	Further, we can conclude
	\small
	\begin{equation}\label{3.3}
	\left\|\mathcal{P}_{\widehat{{\bfU}}_l}\widetilde{{\bfH}}_{k,t} \right\|_F^2 \le \frac{100\mu c_s r}{81n_cn}\ 
	\normalsize \text{and}  
	\ \small \left\|\mathcal{P}_{\widehat{{\bfV}}_l}\widetilde{{\bfH}}_{k,t} \right\|_F^2 \le \frac{100\mu c_s r}{81n_cn}.
	\end{equation}
	\normalsize
	Recall that ${\bfY}=\widetilde{\mathcal{D}}{\bfX}$ and $\widetilde{\mathcal{G}}{\bfY}=\widetilde{\mathcal{H}}{\bf X}$. Define $\widehat{{\bfY}}_l=\widetilde{\mathcal{D}}\widehat{{\bfX}}_l$. Since the measurements are noiseless, then $\bfM=\bfX$ and
	\small
	\begin{equation*}
	\begin{split}
%	\mathcal{P}_{\widehat{\mathcal{S}_l}}
	\widetilde{\mathcal{H}}(\widehat{{\bfX}}_l+\widehat{p}^{-1}\widetilde{\mathcal{P}}_{\Omega_{l+1}}({\bfX}-\widehat{{\bfX}}_l)) =
%	=	\mathcal{P}_{\widehat{\mathcal{S}_l}}
	\widetilde{\mathcal{G}}(\widehat{{\bfY}}_l+\widehat{p}^{-1}\widetilde{\mathcal{P}}_{\Omega_{l+1}}({\bfY}-\widehat{{\bfY}}_l)).
	\end{split}
	\end{equation*}
	\normalsize
	Then,
	\small
	\begin{equation*}
	\begin{split}
	&\left\|\widetilde{{\bfL}}_{l+1}-\widetilde{\mathcal{G}}{\bfY} \right\|_F
	\le 2\left\|\mathcal{P}_{\widehat{\mathcal{S}}_l}\widetilde{\mathcal{G}}(\widehat{{\bfY}}_l+\widehat{p}^{-1}{\mathcal{P}}_{\Omega_{l+1}}({\bfY}-\widehat{{\bfY}}_l))-\widetilde{\mathcal{G}}{\bfY} \right\|_F \\
	\le& 2\left\|\mathcal{P}_{\widehat{\mathcal{S}}_l}\widetilde{\mathcal{G}}{\bfY}-\widetilde{\mathcal{G}}{\bfY} \right\|_F
	+2\left\|\big(\mathcal{P}_{\widehat{\mathcal{S}}_l}\widetilde{\mathcal{G}}-\widehat{p}^{-1}\mathcal{P}_{\widehat{\mathcal{S}}_l}\widetilde{\mathcal{G}}{\mathcal{P}}_{\Omega_{l+1}}\big)({\bfY}-\widehat{{\bfY}}_l) \right\|_F  \\
	=&2\left\|\big({\mathcal{I}}-\mathcal{P}_{\widehat{\mathcal{S}}_l}\big)\widetilde{\mathcal{G}}{\bfY} \right\|_F\\
	&+2\left\|\big(\mathcal{P}_{\widehat{\mathcal{S}}_l}\widetilde{\mathcal{G}}\widetilde{\mathcal{G}}^*-\widehat{p}^{-1}\mathcal{P}_{\widehat{\mathcal{S}}_l}\widetilde{\mathcal{G}}{\mathcal{P}}_{\Omega_{l+1}}\widetilde{\mathcal{G}}^*\big)(\widetilde{{\bfL}}^{\prime}_l-\widetilde{\mathcal{G}}{\bfY}) \right\|_F  \\
	\le&2\left\|\big({\mathcal{I}}-\mathcal{P}_{\widehat{\mathcal{S}}_l}\big)(\widetilde{{\bfL}}^{\prime}_l-\widetilde{\mathcal{G}}{\bfY}) \right\|_F\\
	&+2\left\|\big(\mathcal{P}_{\widehat{\mathcal{S}}_l}\widetilde{\mathcal{G}}\widetilde{\mathcal{G}}^*\mathcal{P}_{\widehat{\mathcal{S}}_l}-\widehat{p}^{-1}\mathcal{P}_{\widehat{\mathcal{S}}_l}\widetilde{\mathcal{G}}{\mathcal{P}}_{\Omega_{l+1}}\widetilde{\mathcal{G}}^*\mathcal{P}_{\widehat{\mathcal{S}}_l}\big)(\widetilde{{\bfL}}^{\prime}_l-\widetilde{\mathcal{G}}{\bfY})  \right\|_F\\
	&+2\left\|\mathcal{P}_{\widehat{\mathcal{S}}_l}\widetilde{\mathcal{G}}({\mathcal{I}}-\widehat{p}^{-1}{\mathcal{P}}_{\Omega_{l+1}})\widetilde{\mathcal{G}}^*({\mathcal{I}}-\mathcal{P}_{\widehat{\mathcal{S}}_l})(\widetilde{{\bfL}}^{\prime}_l-\widetilde{\mathcal{G}}{\bfY})\right\|_F\\ 
	\end{split}
	\end{equation*}
	\normalsize
	\vspace{-5mm}
	\begin{flalign}\label{I_567}
	\vspace{-5mm}
	  :=I_5+I_6+I_7. &&
	\end{flalign}
	where the first inequality comes from (\ref{W_L}).\\
	With (\ref{eqn: t2c2_1}) and (\ref{3.1}), $I_5$ can be bounded as
	\vspace{-1mm}
	\begin{equation}\label{eqn:I_5}
	\vspace{-1mm}
	I_5\le\frac{2\|\widetilde{{\bfL}}^{\prime}_l-\widetilde{\mathcal{G}}{\bfY} \|_F^2 }{\sigma_{\min}(\widetilde{\mathcal{G}}{\bfY})}\le \varepsilon_0\|\widetilde{{\bfL}}_l-\widetilde{\mathcal{G}}{\bfY} \|_F,
	\end{equation}
	As for the item $I_6$, Lemma \ref{condition2} along with (\ref{eqn: t2c2_1}) suggests
	\begin{equation}\label{eqn:I_6}
	\begin{split}
	I_6
	&\le 2\sqrt{\frac{3200\mu c_s r\log(n)}{81\widehat{m}}}\| \widetilde{{\bfL}}^{\prime}_l-\widetilde{\mathcal{G}}{\bfY}\|_F\\
	&\le 16\kappa\sqrt{\frac{3200\mu c_s r\log(n)}{81\widehat{m}}}\| \widetilde{{\bfL}}_l-\widetilde{\mathcal{G}}{\bfY}\|_F 
	\end{split}
	\end{equation}
	with probability at least $1-n_cn^{-2}$. 
	To bound $I_7$,
	\small	
	\begin{equation*}
	\begin{split}
	&\Big({\mathcal{I}}-\mathcal{P}_{\widehat{\mathcal{S}}_l}\Big)\Big(\widetilde{{\bfL}}^{\prime}_l-\widetilde{\mathcal{G}}{\bfY}\Big)
	=\Big({\bfI}-\widehat{{\bfU}}_l\widehat{{\bfU}}_l^*\Big)(-\widetilde{\mathcal{G}}{\bfY})\Big({\bfI}-\widehat{{\bfV}}_l\widehat{{\bfV}}_l^*\Big)\\
	=&\Big(\widetilde{{\bfU}}\widetilde{{\bfU}}^*-\widehat{{\bfU}}_l\widehat{{\bfU}}_l^*\Big)\Big(\widetilde{{\bfL}}^{\prime}_l-\mathcal{\widetilde{G}}{\bfY}\Big)\Big({\bfI}-\widehat{{\bfV}}_l\widehat{{\bfV}}_l^*\Big)\\
	=&\Big(\mathcal{P}_{\widetilde{{\bfU}}}-\mathcal{P}_{\widehat{{\bfU}}_l}\Big)({\mathcal{I}}-\mathcal{P}_{\widetilde{{\bfV}}})\Big(\widetilde{{\bfL}}^{\prime}_l-\mathcal{\widetilde{G}}{\bfY}\Big).
	\end{split}
	\end{equation*}
	\normalsize
Hence, by {Lemma \ref{t2c1}}, with probability at least $1-n_cn^{-2}$,
\footnotesize
\begin{equation}\label{eqn:I_7}
	\begin{split}
	I_7
	&=2\left\|\mathcal{P}_{\widehat{\mathcal{S}}_l}\widetilde{\mathcal{G}}({\mathcal{I}}-\widehat{p}^{-1}{\mathcal{P}}_{\Omega_{l+1}})\widetilde{\mathcal{G}}^* \Big(\mathcal{P}_{\widetilde{{\bfU}}}-\mathcal{P}_{\widehat{{\bfU}}_l}\Big)({\mathcal{I}}-\mathcal{P}_{\widetilde{{\bfV}}})\Big(\widetilde{{\bfL}}^{\prime}_l-\mathcal{\widetilde{G}}{\bfY}\Big)\right\|_F \\
	&\le 2\left\|\mathcal{P}_{\widehat{\mathcal{S}}_l}\widetilde{\mathcal{G}}({\mathcal{I}}-\widehat{p}^{-1}{\mathcal{P}}_{\Omega_{l+1}})\widetilde{\mathcal{G}}^* \Big(\mathcal{P}_{\widetilde{{\bfU}}}-\mathcal{P}_{\widehat{{\bfU}}_l}\Big)\right\| \left\|\widetilde{{\bfL}}^{\prime}_l-\mathcal{\widetilde{G}}{\bfY}\right\|_F\\
	&\le 16\kappa \sqrt{\frac{16000\mu c_s r \log (n)}{81\widehat{m}}}\left\|\widetilde{{\bfL}}^{\prime}_l-\mathcal{\widetilde{G}}{\bfY}\right\|_F.
	\end{split}
\end{equation}
\normalsize
Therefore, if $\widehat{m}\ge C_4\varepsilon_0^{-2}\mu c_s\kappa^2r\log(n)$ for some constant $C_4$,
%\small
\begin{equation*}
\begin{split}
I_6+I_7\le &326\kappa\sqrt{\frac{\mu c_s r \log (n)}{\widehat{m}}}\|\widetilde{{\bfL}}_l-\widetilde{\mathcal{G}}{\bfY} \|_F
	   \le \varepsilon_0\|\widetilde{{\bfL}}_l-\widetilde{\mathcal{G}}{\bfY} \|_F.
\end{split}
\end{equation*}
\normalsize
Putting pieces together gives 
\vspace{-2mm}
\begin{equation}
\vspace{-1mm}
	\begin{split}
	\| \widetilde{{\bfL}}_{l+1}-\widetilde{\mathcal{G}}{\bfY}\|_F
	%&\le\bigg(\varepsilon+326\kappa\sqrt{\frac{\mu c_s r \log (n)}{\widehat{m}}}\bigg)\left\|\widetilde{{\bfL}}_l-\widetilde{\mathcal{G}}{\bfY} \right\|_F \\
	&\le 2\varepsilon_0\|\widetilde{{\bfL}}_l-\widetilde{\mathcal{G}}{\bfY} \|_F 
	\end{split}
\end{equation}
	with probability at least $1-2n_cn^{-2}$. Hence, (\ref{3.1}) also holds when $k={l+1}$.\\
	{\bf Base Case:}
	Since $\widetilde{{\bfL}}_0=\mathcal{Q}_r\big(\widehat{p}^{-1}\widetilde{\mathcal{H}}{\mathcal{P}}_{\Omega_0}({\bfX})\big)$, we can follow the same idea in the proof of base case in Theorem \ref{t1}. Thus, when $k=0$, (\ref{3.1}) is valid with probability at least $1-n_cn^{-2}$ provided $\widehat{m}\ge C_5 \varepsilon_0^{-2}\mu c_s \kappa^6 r^2 \log(n)$
	for some constant $C_5$. 	
	
	Let $C_2=\max\{C_4,C_5\}$. If 	$\widehat{m}\ge C_2 \varepsilon_0^{-2}\mu c_s \kappa^6 r^2 \log(n)$, then for each $l\ge0$, we have
	\begin{equation*}
		\begin{split}
		\| \widetilde{{\bfL}}_{l+1}-\widetilde{\mathcal{G}}{\bfY}\|_F\le 2\varepsilon_0\|\widetilde{{\bfL}}_l-\widetilde{\mathcal{G}}{\bfY} \|_F. 
		\end{split}
	\end{equation*}
	with probability at least $1-2n_cn^{-2}$.
	Directly the following inequality is obtained with probability $1-(2L+1)n_cn^{-2}$,
	\begin{equation}
		\begin{split}
		\| \widetilde{{\bfL}}_L-\widetilde{\mathcal{G}}{\bfY}\|_F\le \nu^{L}\|\widetilde{{\bfL}}_0-\widetilde{\mathcal{G}}{\bfY} \|_F\le\nu^L\frac{\varepsilon_0\sigma_{\min}(\widetilde{\mathcal{G}}{\bfY})}{128\kappa^2}. 
		\end{split}
	\end{equation}
	If we take $L=\Big\lceil \varepsilon_0^{-1}\log \Big(\frac{\sigma_{\max}(\mathcal{H}{\bfX})}{128\kappa^3\varepsilon}\Big)\Big\rceil$ with an arbitrarily small positive constant $\varepsilon$,
	since $\sigma_{\max}(\widetilde{\mathcal{G}}{\bfY})=\sqrt{n_c}\sigma_{\max}(\mathcal{H}{\bfX})$,
	\begin{equation}\label{t2.end}
		 \| \widetilde{{\bfL}}_L-\widetilde{\mathcal{G}}{\bfY}\|_F\le n_c^{1/2}\varepsilon,
	\end{equation}
	which completes the proof of Theorem \ref{t2}.
\end{proof}

\subsection{Proof of Theorem \ref{t3}}
The proof of Theorem \ref{t3} is similar to {Theorem \ref{t2}}, except some modification to handle the noise matrix $\bfN$. We first present the following lemma that will be useful in the proof.
\vspace{-1mm}
\begin{lemma}\label{condition3.1}
	Suppose $m\ge 16\log(n)$, then
	\vspace{-2mm}
	\begin{equation*}
	\left\|p^{-1}\mathcal{\widetilde{H}}{\mathcal{P}}_{\Omega}({\bfN})-\widetilde{\mathcal{H}}{\bfN} \right\|\le \displaystyle \sqrt{\frac{16\log(n)}{m}}n_cn\left\| \widetilde{\mathcal{H}}{\bfN} \right\|_{\infty}
	\end{equation*} 
	with probability at least $1-n_cn^{-2}$.
\end{lemma}
%\input{proof_condition3.1.tex}
\begin{proof}[Proof of Theorem \ref{t3}]
	For the noisy case where $\bfM=\bfX+\bfN$, we have assumed $ \left\|\bfN \right\|_{\infty}\le\displaystyle
	\frac{\varepsilon_0\left\|\mathcal{H} \bfX\right\|}{2048\kappa^3r^{1/2}n_c^{1/2}n}$. Recall \eqref{y_l}, define $\bfS=\widetilde{\mathcal{D}}\bfN$, then  
	\vspace{-2mm}
	\begin{equation*}
	\begin{split}
	   \| \widetilde{\mathcal{G}}\bfS\|_{\infty}
	 =&\| \widetilde{\mathcal{H}}\bfN\|_{\infty}=\left\| \bfN\right\|_{\infty}
	\le\frac{\varepsilon_0 \sigma_{\min}(\widetilde{\mathcal{G}}\bfY)}{2048\kappa^2r^{1/2}n_cn}.
	\end{split}
	\end{equation*}
	Similar to the derivation of (\ref{W_L}), we have
	\small
	\begin{equation*}
	\begin{split}
		   &\|\widetilde{{\bfL}}_{l+1}-\widetilde{\mathcal{G}}{\bfY} \|
		\le 2\left\|\mathcal{P}_{\widehat{\mathcal{S}}_l}\widetilde{\mathcal{G}}(\widehat{{\bfY}}_l+\widehat{p}^{-1}{\mathcal{P}}_{\Omega_{l+1}}({\bfY}+\bfS-\widehat{{\bfY}}_l))-\widetilde{\mathcal{G}}{\bfY} \right\|\\
		\le& 2\left\|\mathcal{P}_{\widehat{\mathcal{S}}_l}\widetilde{\mathcal{G}}(\widehat{{\bfY}}_l+\widehat{p}^{-1}{\mathcal{P}}_{\Omega_{l+1}}({\bfY}-\widehat{{\bfY}}_l))-\widetilde{\mathcal{G}}{\bfY} \right\|\\
		   &+2\|\widehat{p}^{-1}\mathcal{P}_{\widehat{\mathcal{S}}_l}\widetilde{\mathcal{G}} {\mathcal{P}}_{\Omega_{l+1}}(\bfS)\|. 
	\end{split}
	\end{equation*}
%	\normalsize
%	Immediately,
%	\small
	\begin{equation*}
		\begin{split}
		&\|\widetilde{{\bfL}}_{l+1}-\widetilde{\mathcal{G}}{\bfY} \|_F\le\sqrt{2r}\|\widetilde{{\bfL}}_{l+1}-\widetilde{\mathcal{G}}{\bfY} \|\\
		\le& 2\sqrt{2r}\left\|\mathcal{P}_{\widehat{\mathcal{S}}_l}\widetilde{\mathcal{G}}(\widehat{{\bfY}}_l+\widehat{p}^{-1}{\mathcal{P}}_{\Omega_{l+1}}({\bfY}+\bfS-\widehat{{\bfY}}_l))-\widetilde{\mathcal{G}}{\bfY} \right\|\\
		\le& 2\sqrt{2r}\left\|\mathcal{P}_{\widehat{\mathcal{S}}_l}\widetilde{\mathcal{G}}(\widehat{{\bfY}}_l+\widehat{p}^{-1}{\mathcal{P}}_{\Omega_{l+1}}({\bfY}-\widehat{{\bfY}}_l))-\widetilde{\mathcal{G}}{\bfY} \right\|\\
		&+2\sqrt{2r}\|\widehat{p}^{-1}\mathcal{P}_{\widehat{\mathcal{S}}_l}\widetilde{\mathcal{G}} {\mathcal{P}}_{\Omega_{l+1}}(\bfS)\|\\
		\le	&2\sqrt{2r}\left\|\big({\mathcal{I}}-\mathcal{P}_{\widehat{\mathcal{S}}_l}\big)(\widetilde{{\bfL}}^{\prime}_l-\widetilde{\mathcal{G}}{\bfY}) \right\|_F\\
		&+2\sqrt{2r}\left\|\big(\mathcal{P}_{\widehat{\mathcal{S}}_l}\widetilde{\mathcal{G}}\widetilde{\mathcal{G}}^*\mathcal{P}_{\widehat{\mathcal{S}}_l}-\widehat{p}^{-1}\mathcal{P}_{\widehat{\mathcal{S}}_l}\widetilde{\mathcal{G}}{\mathcal{P}}_{\Omega_{l+1}}\widetilde{\mathcal{G}}^*\mathcal{P}_{\widehat{\mathcal{S}}_l}\big)(\widetilde{{\bfL}}^{\prime}_l-\widetilde{\mathcal{G}}{\bfY})  \right\|_F\\
		&+2\sqrt{2r}\left\|\mathcal{P}_{\widehat{\mathcal{S}}_l}\widetilde{\mathcal{G}}({\mathcal{I}}-\widehat{p}^{-1}{\mathcal{P}}_{\Omega_{l+1}})\widetilde{\mathcal{G}}^*({\mathcal{I}}-\mathcal{P}_{\widehat{\mathcal{S}}_l})(\widetilde{{\bfL}}^{\prime}_l-\widetilde{\mathcal{G}}{\bfY})\right\|_F\\		
		&+2\sqrt{2r}\|\widehat{p}^{-1}\mathcal{P}_{\widehat{\mathcal{S}}_l}\widetilde{\mathcal{G}} {\mathcal{P}}_{\Omega_{l+1}}(\bfS)\|
%		:=& \sqrt{2r}(I_5+I_6+I_7)+I_9, 
		\end{split}
		\end{equation*}	
		\normalsize
		\vspace{-4.5mm}
		\begin{flalign}\label{t4.I_5}
		:=\sqrt{2r}(I_5+I_6+I_7)+I_9, &&
		\end{flalign}	
	where $I_5+I_6+I_7$ has been defined in \eqref{I_567}.\\
	Similar to the proof of {Theorem \ref{t2}}, we show that the following inequality holds with high probability by induction.
	\vspace{-2mm}
%	\small
		\begin{equation}\label{4.1}
		\|\widetilde{{\bfL}}_k-\widetilde{\mathcal{G}}{\bfY}\|_F\le\frac{\varepsilon_0\sigma_{\min}(\widetilde{\mathcal{G}}{\bfY})}{128\sqrt{2}\kappa^2r^{1/2}}. 
		\end{equation}
		\normalsize	
		{\bf Inductive Step:} Suppose (\ref{4.1}) holds when $k=l$ and $l\ge0$. 
		By {Lemma \ref{sub1} } and (\ref{3.1}), we have
%		\small
		\begin{equation*}
		\begin{split}
		\sqrt{2r}I_5
		\le&\frac{2\sqrt{2r}\|\widetilde{{\bfL}}^{\prime}_l-\widetilde{\mathcal{G}}{\bfY} \|_F^2 }{\sigma_{\min}(\widetilde{\mathcal{G}}{\bfY})}
		\le \frac{128\sqrt{2}\kappa^2\sqrt{r}\|\widetilde{{\bfL}}_l-\widetilde{\mathcal{G}}{\bfY} \|_F^2 }{\sigma_{\min}(\widetilde{\mathcal{G}}{\bfY})}\\
		\le& \varepsilon_0\|\widetilde{{\bfL}}_l-\widetilde{\mathcal{G}}{\bfY} \|_F.
		\end{split}
		\end{equation*}
		\normalsize
		Similar to $I_6$ and $I_7$,
		\vspace{-2mm}
		\begin{equation*}
		\begin{split}
		\sqrt{2r}(I_6+I_7)
		\le &326\kappa\sqrt{\frac{2\mu c_s r^2 \log (n)}{\widehat{m}}}\|\widetilde{{\bfL}}_l-\widetilde{\mathcal{G}}{\bfY} \|_F.
		\end{split}
		\end{equation*}
		Hence, if $\widehat{m}\ge C_6\varepsilon_0^{-2}\mu c_s\kappa^2r^2\log(n)$ for some constant $C_6$, 
		\begin{equation*}
		\begin{split}
		\sqrt{2r}(I_5+I_6+I_7)&\le 2\varepsilon_0\|\widetilde{{\bfL}}_l-\widetilde{\mathcal{G}}{\bfY} \|_F 
		\end{split}
		\end{equation*}
		with probability at least $1-2n_cn^{-2}$.
		On the other hand, if $m\ge 256r\log(n)$, then with probability at least $1-n_cn^{-2}$
		\vspace{-1mm}
		\begin{equation}\label{I_9}
		\begin{split}
		\vspace{-3mm}
		I_9\le&2\sqrt{2r}\|\widehat{p}^{-1}\widetilde{\mathcal{G}} {\mathcal{P}}_{\Omega_{l+1}}(\bfS)\|\\
		\le&2\sqrt{2r}\|\widehat{p}^{-1}\widetilde{\mathcal{G}} {\mathcal{P}}_{\Omega_{l+1}}(\bfS)-\widetilde{\mathcal{G}}\bfS\|+2\sqrt{2r}\| \widetilde{\mathcal{G}}\bfS\| \\
		\le&8\sqrt{2}\sqrt{\frac{r\log(n)}{m}}n_cn\|\widetilde{\mathcal{G}}\bfS \|_{\infty}+2\sqrt{2r}n_cn\|\widetilde{\mathcal{G}}\bfS \|_{\infty}\\
		\le&\frac{1}{16\sqrt{2}}\sqrt{\frac{r\log(n)}{m}}\frac{\varepsilon_0\sigma_{\min}(\widetilde{\mathcal{G}}\bfY)}{\kappa^2r^{1/2}}+\frac{\varepsilon_0\sigma_{\min}(\widetilde{\mathcal{G}}{\bfY})}{512\sqrt{2}\kappa^2r^{1/2}}\\
		\le&\frac{\varepsilon_0\sigma_{\min}(\widetilde{\mathcal{G}}{\bfY})}{256\sqrt{2}\kappa^2r^{1/2}},
		\end{split}
		\end{equation}
		\normalsize
		where the second last inequality comes from {Lemma \ref{condition3.1}}.\\
		Following  $\nu=2\varepsilon_0\le1/2$ and (\ref{4.1}), with probability at least $1-3n_cn^{-2}$, we can bound $\|\widetilde{{\bfL}}_{l+1}-\widetilde{\mathcal{G}}{\bfY} \|_F$ by
		\begin{equation*}
		\begin{split}
%		\|\widetilde{{\bfL}}_{l+1}-\widetilde{\mathcal{G}}{\bfY} \|_F
%		\le&
		\frac{1}{2}\|\widetilde{{\bfL}}_{l}-\widetilde{\mathcal{G}}{\bfY} \|_F+\frac{\varepsilon_0\sigma_{\min}(\widetilde{\mathcal{G}}{\bfY})}{256\sqrt{2}\kappa^2r^{1/2}}
		\le\frac{\varepsilon_0\sigma_{\min}(\widetilde{\mathcal{G}}{\bfY})}{128\sqrt{2}\kappa^2r^{1/2}}.
		\end{split}
		\end{equation*}
		Hence, (\ref{4.1}) also holds when $k={l+1}$.
		
\noindent{\bf Base Case:}
		Since $\widetilde{{\bfL}}_0=\mathcal{Q}_r\big(\widehat{p}^{-1}\widetilde{\mathcal{H}}{\mathcal{P}}_{\Omega_0}({\bfX+\bfN})\big)$, then with probability at least $1-n_cn^{-2}$,
		\small
		\begin{equation*}		
		\begin{split}
		&\|\widetilde{{\bfL}}_0-\mathcal{\widetilde{G}}{\bfY}\|_F\le\sqrt{2r}\|\widetilde{{\bfL}}_0-\mathcal{\widetilde{G}}{\bfY}\|\\
		\le&\sqrt{2r}\left\|p^{-1}\mathcal{\widetilde{G}}\mathcal{P}_{\Omega}({\bfY}+\bfS)-\widetilde{{\bfL}}_0\right\|
		+\sqrt{2r}\left\|p^{-1}\mathcal{\widetilde{G}}\mathcal{P}_{\Omega}({\bfY}+\bfS)-\mathcal{\widetilde{G}}{\bfY}\right\|\\
		\le& 2\sqrt{2r}\left\|p^{-1}\mathcal{\widetilde{G}}\mathcal{P}_{\Omega}({\bfY})-\mathcal{\widetilde{G}}{\bfY}\right\|+2\sqrt{2r}\left\| p^{-1}\mathcal{\widetilde{G}}\mathcal{P}_{\Omega}({\bfS})\right\|\\
		\le&\sqrt{\frac{512\mu c_sr^2\log(n)}{m}}\|\mathcal{\widetilde{G}}{\bfY}\|+\frac{\varepsilon_0\sigma_{\min}(\widetilde{\mathcal{G}}{\bfY})}{256\sqrt{2}\kappa^2\sqrt{r}}.
		\end{split}		
		\end{equation*}
		\normalsize
		where the last inequality comes from $(\ref{I_9})$ and {Lemma \ref{condition3}}.
		To guarantee that (\ref{4.1}) holds with $k=0$, we need 
%		\vspace{-2mm}
%		\begin{equation*}
%		\vspace{-2mm}
%		\|\widetilde{{\bfL}}_0-\mathcal{\widetilde{G}}{\bfY}\|_F\le\frac{\varepsilon_0\sigma_{\min}(\widetilde{\mathcal{G}}{\bfY})}{128\sqrt{2}\kappa^2\sqrt{r}},
%		\end{equation*}  
%		we need
		\begin{equation}
		\sqrt{\frac{512\mu c_sr^2\log(n)}{m}}\|\mathcal{\widetilde{G}}{\bfY}\|\le\frac{\varepsilon_0\sigma_{\min}(\widetilde{\mathcal{G}}{\bfY})}{256\sqrt{2}\kappa^2\sqrt{r}}.
		\end{equation}
		That is 
		$\widehat{m}\ge C_7 \varepsilon_0^{-2}\mu c_s \kappa^6 r^3 \log(n)$ for some constant $C_7$.	
			
		Let $C_3=\max\{C_6,C_7\}$, if $\widehat{m}\ge C_3 \varepsilon_0^{-2}\mu c_s \kappa^6 r^3 \log(n)$, for each $l\ge0$, with probability $1-2n_cn^{-2}$, we have
		\vspace{-1mm}
		\begin{equation}
		\vspace{-1mm}
		\begin{split}
		\| \widetilde{{\bfL}}_{l+1}-\widetilde{\mathcal{G}}{\bfY}\|_F\le &2\varepsilon_0\|\widetilde{{\bfL}}_l-\widetilde{\mathcal{G}}{\bfY} \|_F+\Delta. 
		\end{split}
		\end{equation}
		where $\Delta=32\sqrt{2}n_cn\|\widetilde{\mathcal{G}}\bfS \|_{\infty}+2\sqrt{2}r^{1/2}\|\widetilde{\mathcal{G}}\bfS \|$. Then
		\begin{equation*}
		\begin{split}
		\| \widetilde{{\bfL}}_{l+1}-\widetilde{\mathcal{G}}{\bfY}\|_F-\frac{\Delta}{1-\nu}\le \nu\Big(\|\widetilde{{\bfL}}_l-\widetilde{\mathcal{G}}{\bfY} \|_F-\frac{\Delta}{1-\nu}\Big). 
		\end{split}
		\end{equation*}
		\normalsize
		Therefore, with probability $1-(3L+1)n_cn^{-2}$, 
		\begin{equation}
		\begin{split}
		\| \widetilde{{\bfL}}_L-\widetilde{\mathcal{G}}{\bfY}\|_F&\le \nu^{L}\|\widetilde{{\bfL}}_0-\widetilde{\mathcal{G}}{\bfY}\|_F+\frac{\Delta}{1-\nu}.
		\end{split}
		\end{equation}
		Similar to \eqref{t2.end}, take $L=\Big\lceil \varepsilon_0^{-1}\log \Big(\frac{\sigma_{\max}(\mathcal{H}{\bfX})}{128\kappa^3\varepsilon}\Big)\Big\rceil$ with an arbitrarily small positive constant $\varepsilon$,
		since $\nu\le1/2$,
		\begin{equation*}
		\begin{split}
		\| \widetilde{{\bfL}}_L-\widetilde{\mathcal{G}}{\bfY}\|_F
		\le& {n}_c^{1/2}\varepsilon+64\sqrt{2}n_cn\|\widetilde{\mathcal{G}}\bfS \|_{\infty}+4\sqrt{2}r^{1/2}\|\widetilde{\mathcal{G}}\bfS \|\\
		\le& {n}_c^{1/2}\varepsilon+128n_cn\|\widetilde{\mathcal{G}}\bfS \|_{\infty}+8{r}^{1/2}\|\widetilde{\mathcal{G}}\bfS \|.
		\end{split}
		\end{equation*}
		which completes the proof of {Theorem \ref{t3}}.
\end{proof}



==> chapter_3/TNNLS-2019-P-12087-Relate.tex <==
\section{Related works}
With development and success of neural network,  understanding the deep reasons behind the performance of neural network becomes a popular topic. 
However, it is impossible for us to review previous works due to the rapid growth of neural network, so below we only focus on the most relevant works with this chapter.  

From the prospective of non-convex optimization, the success of gradient-based algorithm is also observed in other fields, like low-rank matrix completion (MC) problems\cite{WCCL16, JN15, ZHWC18}. Recent work \cite{GLM16,BNS16,PKC16} in MC pointed out all the local minima can be escaped or are global minima by factorizing the target matrix, though MC involves solving a non-convex problem. Inspired by the success in MC, more work begin to explore the theoretical performance of neural network. However, due to variety and complexity in the structure of neural network, studying the performance of neural network over all cases leads to quite negative results. 
For example, the authors in \cite{Sh18} claimed some nice properties, including but not limited to smoothness and incoherence, should be captured by the distribution of the input data or the output function $g$ in \eqref{eqn: major_equ}. 
Also, ref. \cite{BG17} pointed out that training a non-overlapping convolutional neural network is NP-hard.  
Moreover, even under the assumption of Gaussian input, the authors in \cite{SS17} showed spurious local minima exists for neural network with multiple nodes, $K> 6$, in the hidden layer. 

Therefore, current works focused more on neural network with simple structure and a group of nice input distributions. Only \cite{LSL18} provided the analysis of global convergence for multiple layer neural network by adding one exponential node in each layer, however, the assumption in \cite{LSB09} requires the objective function to be at least twice differentiable and thus smooth as well.  There is no theoretical guarantee for the sampling complexity in \cite{LSB09}, either. By adding additional regularization to the population risk function of \eqref{eqn: sample_risk} for one-hidden layer neural network, the authors in  \cite{GLM17} claimed that the regularized objective function has a good landscaped that all local minima are global optimal and the global optimal is corresponding with the ground truth as well. However, the computational complexity of \cite{GLM17} is a polynomial function of  $1/\varepsilon$, where $\varepsilon$ is the approximation error, so the algorithm in \cite{GLM17} is only sub-linear. Though sampling complexity is also discussed in \cite{GLM17}, the sampling complexity depends on a polynomial function of $d$ while the degree freedom of $\bfW^*$ is a linear function of $d$. When it turns to one-hidden layer neural network with one node, all these work \cite{Tian17,BG17,DLTPS17} provided linear convergence to the global optimal through random initialization. The analysis of such simplest neural network showed that the basin of attraction near the global optimal is significant large that random initial point lies in this region with a constant probability.

However, when moving into one-hidden layer neural network structure but with multiple nodes, the landscape analysis become hard. Ref. \cite{GLM17} pointed out that the landscape of $f(\bfW)$ itself has significant number of spurious local minima, and similar result is also suggested in \cite{SS17}. 
More importantly, with finite samplings, the landscape of empirical risk function $\hat{f}_N$  suffers from bad properties, like non-smoothness and non-deterministic, even under the assumption of Gaussian distribution input. Thus, 
there is another line of research that relied on well-designed initialization and analysis of the local landscape near the initial point.   
The tensor initialization method is first presented in \cite{ZSD17}, and it relies on the preliminary knowledge of the input distribution to provide a good initial point that is reasonable close to the global optimal.  Built upon the tensor initialization method , 
several recent works \cite{FCL18, ZSD17, ZSJB17, ZYWG18}  provides the linear convergence and sampling complexity that almost linearly depends on $d$ for certain setup of one-hidden layer neural networks with multiple nodes. 
Ref. \cite{FCL18} considered the classification problem as the output $y$ is quantized as $ 0$ or $1$, while the other three works focused on regression problems. 
Ref. \cite{ZSJB17} mainly focused on fully connected neural network problem with smooth active function. In contrast, ref. \cite{ZYWG18} analyzed the fully connected neural network
 with ReLU active function. Among the four works, ref. \cite{ZSD17} is the most relevant work with this chapter since we both built upon the tensor initialization algorithm and consider non-overlapping convolutional neural network. However, the convergence analysis of \cite{ZSD17} relied on the smoothness of objective function $\hat{f}_N$  and thus cannot handle the non-smooth active function, ReLU, in its major theorem (Theorem 5.1, \cite{ZSD17}). Instead, we first analyze the convergence of population risk function $f(\bfW)$ which is a smooth function for ReLU, and then the analysis of $\hat{f}_N$ is given in terms of the error bound between $f$ and $\hat{f}_N$. Therefore, by such roadmap of proof, we offered the linear convergence of global convergence with a nearly optimal sampling complexity. 
 
 %we also focused on regression problem and limited our work to the most widely-used active function named ReLU. However, as a non-smooth active function, ref. \cite{ZSD17} lacked the comprehensive analysis for ReLU, which can be found in the paragraph before Theorem 5.1 in \cite{ZSD17}, and the major theorem Theorem 5.1 in \cite{ZSD17} excludes the case of non-smooth active function. 
 
%Another line of research focused on analyzing the landscape of the non-convex objective function in neural network problem. Such work do not rely on well-designed initialization or just use random initialization, however, the analysis of global convergence is limited to either one or two nodes in the hidden layer or some special structures of neural network.  
%For neural network with one node in the hidden layer, like $K=1$ in \eqref{eqn: major_equ}, refs. \cite{BG17, DLT17} showed that the iterates converged to the ground truth linearly with a constant probability by random initialization. However, for neural network with multiple nodes in the hidden layer, ref. \cite{SS17} pointed out the spurious local minima is fairly common.
 
None of the previous works above provide a theoretical analysis for accelerated gradient descent method.  
In convex setting, accelerated gradient descent methods are widely applied  to speed up the rate of convergence and thus reduce the number of iterations. NAG method in \cite{Nesterov13} and HB method in \cite{P87} are the most popular AGD algorithms. 
The update rule of HB method is given as 
%\begin{equation}
%	\bfW_{k+1} = \bfW_k - \eta \nabla f\big(\bfW_k+\beta(\bfW_k -\bfW_{k-1})\big)+\beta(\bfW_k -\bfW_{k-1}),
%\end{equation}
%while the update rule of HB is given as 
\begin{equation}\label{eqn: update_HB}
\bfW_{k+1} = \bfW_k - \eta \nabla f(\bfW_k)+\beta(\bfW_k -\bfW_{k-1}),
\end{equation}
where $\eta$ is the step size of first-order gradient descent and $\beta$ is the momentum parameter.
The update rule of NAG method is similar to \eqref{eqn: update_HB} but the gradient is calculated in $\bfW_k+ \beta(\bfW_k -\bfW_{k-1})$ instead of $\bfW_k$.
Though \eqref{eqn: optimization_problem} is a non-convex optimization problem in general, the effectiveness of AGD methods in solving neural network problems are verified in
\cite{SMDH13} numerically.
 %and the numerical results in \cite{SMDH13} showed that AGD method could achieve the similar convergence rate and recovery error as some second-order algorithms in deep neural network problems. 
However, there is no convergence analysis in \cite{SMDH13}.
Consider other settings of non-convex problems,
ref. \cite{ZHWC18} showed a small positive momentum parameter $\beta$ could accelerate the convergence rate in low-rank matrix completion problem. Instead, ref. \cite{XCHZ18} provides the region of $(\eta, \beta)$ that guarantee linear convergence under Regularity Condition. 

%As a typical non-convex problems, the optimization problems of neural networks suffered from fake local minima. 
%From the perspective of non-convex optimization, the success of gradient-based algorithm in neural network is not a special case.  
%Throughout the decade, several gradient-based algorithms has been proved to be able to solving the non-convex optimization problem in the filed of low-rank matrix completion. 
%Some works relied on well-designed initialization and showed the local convexity around the initial point \cite{WCCL16, JN15, ZHWC18}.  
%Under some mild conditions, it has been proved that there is no spurious local minima universally in low-rank matrix completion problems \cite{GJZ17,GLM16,BNS16,PKC16}. 

%Besides vanilla GD algorithm, AGD comes to attention of researchers in solving non-convex problems.

%Back to neural networks problems,some works focused on analyzing the landscape of the objective function. However, for multiple nodes, like when $K>2$, limited results are presented. Also, some work even pointed out there are many local minima when multiple nodes. 




==> chapter_6/algorithm.tex <==
\subsection{Algorithm}\label{sec: algorithm}
We consider an iterative self-training method such as \citep{Lee13}, which can be divided into   steps: 



\begin{enumerate}
    \item Initial $\ell =0$ and obtain a  model $\W[\ell]$, denoted as the teacher model,   using labeled data $\mathcal{D}$ only;
%\noindent   For $\ell = 0 , 1, \cdots, L-1$
    \item Use the teacher model    to calculate  pseudo labels $\w[y]_m$ of unlabeled data in $\w[\mathcal{D}]$. %=\{\w[\bfx]_m \}_{m=1}^M$. 
    \item Train the neural network by solving (\ref{eqn: empirical_risk_function}) %via minimizing the objective function as shown in \eqref{eqn: empirical_risk_function} 
    via $T$-step  mini-batch stochastic gradient descent method using disjoint subsets $\{\mathcal{D}_t\}_{t=0}^{T-1}$ and $\{\widetilde{\mathcal{D}}_t\}_{t=0}^{T-1}$. Let $\W[\ell]$ denote the obtained student model. 
    \item Use $\W[\ell]$ as the current teacher model. Let $\ell=\ell+1$ and go back to step 2.
\end{enumerate}
The pseudocode of the self-training method is summarized in Algorithm
\ref{Algorithm: Alg1}.
\begin{algorithm}[h]
	\caption{Mini-batch stochastic gradient Descent Algorithm}\label{Algorithm: Alg1}
	\begin{algorithmic}
		\State \textbf{Input:} labeled $\mathcal{D}=\{(\bfx_n, y_n) \}_{n=1}^{N}$,  
		 unlabeled data $\w[\mathcal{D}]=\{\widetilde{\bfx}_m \}_{m=1}^{M}$,
		gradient step size $\eta$;
		\State \textbf{Initialization:} preliminary teacher model with weights $\bfW^{(0)}$;
		\State \textbf{Partition:} divide $\mathcal{D}$ and $\widetilde{\mathcal{D}}$ into $T$ disjoint subsets $\{ \mathcal{D}_t \}_{t=0}^{T-1}$ and $\{\widetilde{\mathcal{D}}_t\}_{t = 0}^{T-1}$, respectively; \For{$\ell = 0 , 1, \cdots, L-1$}
		    \State 1. Use the estimated teacher model $\bfW^{(\ell)}$ to generate pseudo labels for $\{\widetilde{\bfx}_m\}_{m=1}^M$:
		    \State \qquad $y_m = g(\bfW^{(\ell)};\w[\bfx]_m)$ for $m =1, 2, \cdots, M$;
		    \State 2. Obtain the student model ${\bfW}$ through minimizing \eqref{eqn: empirical_risk_function} via  mini-batch stochastic gradient descent method using $\mathcal{D}_t$ and $\widetilde{\mathcal{D}}_t$;
		    \State 3. Update the new teacher model  as the obtained student model: \qquad $\bfW^{(\ell+1)} = \bfW$;
		 \EndFor
	\end{algorithmic}
\end{algorithm}

